On Simple Mechanisms for Dependent Items

We study the problem of selling $n$ heterogeneous items to a single buyer, whose values for different items are dependent. Under arbitrary dependence, Hart and Nisan show that no simple mechanism can achieve a non-negligible fraction of the optimal revenue even with only two items. We consider the setting where the buyer's type is drawn from a correlated distribution that can be captured by a Markov Random Field, one of the most prominent frameworks for modeling high-dimensional distributions with structure. If the buyer's valuation is additive or unit-demand, we extend the result to all MRFs and show that max(SRev,BRev) can achieve an $\Omega\left(\frac{1}{e^{O(\Delta)}}\right)$-fraction of the optimal revenue, where $\Delta$ is a parameter of the MRF that is determined by how much the value of an item can be influenced by the values of the other items. We further show that the exponential dependence on $\Delta$ is unavoidable for our approach and a polynomial dependence on $\Delta$ is unavoidable for any approach. When the buyer has a XOS valuation, we show that max(Srev,Brev) achieves at least an $\Omega\left(\frac{1}{e^{O(\Delta)}+\frac{1}{\sqrt{n\gamma}}}\right)$-fraction of the optimal revenue, where $\gamma$ is the spectral gap of the Glauber dynamics of the MRF. Note that in the special case of independently distributed items, $\Delta=0$ and $\frac{1}{n\gamma}\leq 1$, and our results recover the known constant factor approximations for a XOS buyer. We further extend our parametric approximation to several other well-studied dependency measures such as the Dobrushin coefficient and the inverse temperature. Our results are based on the Duality-Framework by Cai et al. and a new concentration inequality for XOS functions over dependent random variables.

==> MRF/3-wise.tex <==
In this section we are going to show that if we do not restrict our MRF to pairwise potentials,
then some counter intuitive things can happen.


\begin{lemma}
Let the type distribution $D$ be generated by a MRF with pairwise potentials.
Let the highest possible Markov Correlation be $\beta$.
That is $\beta = \max_{i,j \in [n]}\beta_{i,j}$.


For any value $\beta'$,
we can create a MRF $D'$ with $n + \left\lceil \frac{\beta}{\beta'} \right\rceil$ items with 3-way potentials (that means that the potentials in $D'$ have exactly 3 inputs) that has the same joint distribution as $D$ with respect to the $n$ common items and the rest $\left\lceil \frac{\beta}{\beta'} \right\rceil$ contain exactly one type.
\end{lemma}


\begin{proof}
Let $G=([n],E)$ be the graph associated with $D$.
First we are going to describe the graph $G'=([n + \left\lceil \frac{\beta}{\beta'} \right\rceil],E')$ associated with $D'$.
For $i\leq n$, we couple the $i$-th item of $D'$ with the $i$-th item of $D$.
From now on we refer to the first $n$ items of $D'$ as valuable items and to the rest of items as auxiliary items.


Now we are going to define the 3-wise potentials.
Let $e=(i,j,k)\in E'$,
then $i,j \in [n]$ and $k >n$.
That means that the hyperedges of the graph have two endpoints exactly in the set of the valuable items and one endpoint in the auxiliary items.
We use the same unitwise potentials for the valuable items as the unitwise potentials in $D$ and for the auxiliary items we define unitwise potential equal to $1$.


Since we assumed that the auxiliary items have only one type,
we can recreate any value of the pairwise potential between types $t_i \in T_i$ and $t_j \in T_j$ in $D$ with the $\left\lceil \frac{\beta}{\beta'} \right\rceil$ possible 3-wise potentials that connects a hyperedge that contain this specific pair of nodes with any auxiliary item.
Since the we assumed that $\beta'$ is the maximum possible value of any 3-wise potential,
the claim holds.

The statement follows by noting that since the valuable items share the same unitwise potentials as the items in $D$ and for each $e\in E$ we have recreated the value of the pairwise potentials with the 3-way potentials.
\end{proof}




==> MRF/3_wise_potentials.tex <==
\subsection{Impossibility of Approximation when dealing with 3-wise Potentials}


In this section we are going to show that when we the buyer valuation is defined over a hypergraph,
then we cannot hope to approximate the optimal revenue with simple mechanisms that do not depend on a a combination of the the number of items and the highest value of any potential.


\begin{lemma}\label{lem:3_wise}
Let the type distribution $D$ be generated by a MRF over a simple graph $G(V,E)$.
Let the highest possible value of any potential be $\beta$,
that is $\max_{e\in E, \vT \in T}|\psi_e(\vT_e)|\leq \beta$.


For any value $\beta'$,
we can create a MRF $D'$ over a hypergraph $G'=(V', E')$ with 3-way potentials (that means that the potentials in $D'$ have exactly 3 inputs),
where $|V'|= n + \left\lceil \frac{\beta}{\beta'} \right\rceil$
and the highest value of any potential is $\beta'$ ($\max_{e\in E', \vT' \in T'}|\psi_e(\vT_e')|\leq \beta'$)
that has the same joint distribution as $D$ with respect to the $n$ common items and the rest $\left\lceil \frac{\beta}{\beta'} \right\rceil$ contain exactly one type.
\end{lemma}


\begin{proof}
Let $G=([n],E)$ be the graph associated with $D$.
First we are going to describe the graph $G'=([n + \left\lceil \frac{\beta}{\beta'} \right\rceil],E')$ associated with $D'$.
For $i\leq n$, we couple the $i$-th item of $D'$ with the $i$-th item of $D$.
From now on we refer to the first $n$ items of $D'$ as valuable items and to the rest of items as auxiliary items.
Since the auxiliary items contain exactly one type,
we are going to omit their type.


For each valuable item $i$,
the potential $\psi_i(\cdot)$ in $D'$ is the same as the potential $\psi_i(\cdot)$ in $D$.
For each auxiliary item $j$,
we define the potential $\psi_j(\cdot)=1$.
We are going to prove that for each $e\in E$ and $\vT \in T$,
we have that $\psi_e(\vT_e) = \sum_{e'\in E': e \subset e'}\psi_{e'}(\vT_{e'})$.
The combination of those two things implies that the joint distribution of the valuable items of $D'$ is the same as the distribution of $D$.


Now we are going to define the 3-wise potentials of $D'$.
For each $e'=(i,j,k)\in E'$,
$i,j \in [n]$ and $k >n$.
That means that the hyperedges of the graph have two endpoints exactly in the set of the valuable items and one endpoint in the auxiliary items.
%For any $e=(i,j)\in E$,
%$|\psi_e(\vT)|\leq \beta$.
%For each of the auxiliary item $k$ ,
%there exists $e'=(i,j,k) \in E'$.
Therefore for each $e=(i,j)\in E$,
$|\{e'\in E': e \subset e'\}|=\left\lceil\frac{\beta}{\beta'} \right\rceil$.
Since for each $e'\in E'$ we have $|\psi_e'(\vT)|\leq \beta'$ and for each $e\in E$ we also have $|\psi_e(\vT)|\leq \beta$,
we can couple the values of $\psi_e'(\cdot)$,
such that for each $e \in E $ and $\vT \in T$ we have $\psi_e(\vT) = \sum_{e' \in E' : e \subset e'}\psi_{e'}(\vT)$.


Therefore the joint distirbution of $D'$ and $D$ is the same w.r.t. the valuable items.

\end{proof}




When dealing with pairwise potentials (which means that the buyer valuation is generated by MRF over a simple graph),
simple mechanisms are within a multiplicative factor approximation that could depend on the value of the highest Markov Correlations or on the number of item.
Since Lemma~\ref{lem:3_wise} let us reduce an instance of a MRF $D$ with pairwise potential,
such that the highest potential is $\beta$ and the number of items $n$,
to an instance where the buyer valuation is generated by a MRF $D'$ over a hypergraph,
but with arbitrary small highest potential and more items,
we can infer that the approximation ratio of a simple mechanism to the optimal one,
depends both on the value of the highest potential and the number of items.

==> MRF/LB_copies.tex <==
\section{Lower Bound for the Copies Setting}\label{sec:LB_copies}

We consider a valuation that is generated by a MRF $D$,
and we prove that the optimal revenue in the COPIES settings can be exponential in $\Delta(\vT)$, while both $\srev$ and $\brev$ are less than $2$. Indeed, we prove an even stronger result that the gap is exponential in the inverse temperature, which is an upper bound of $\Delta(\vT)$.


\begin{prevproof}{Theorem}{thm:COPIES_example}
We construct the MRF in the following way.
The first item has support $T_1=\{2^0,2^1,2^2,\ldots,2^{k^n-1}\}$,
where $k\in \mathbb{N}$ is going to be defined later.
Let $\epsilon_1,\ldots,\epsilon_k$ be some tiny values,
the support for the other items is $T_r=\{\epsilon_i\}_{i\in[k]}$.
We consider the following node potential for the first item:
\begin{align*}
    \psi_1(2^i) =
    \begin{cases}
    \ln(\frac{1}{2^{i+1}}) \quad &\text{if $0 \leq i \leq k^n-2$} \\
    \ln(\frac{1}{2^{i}}) & \text{if $i = k^n-1$}
    \end{cases}
\end{align*}

The node potentials for the other items is:

\begin{align*}
    \psi_i (a) =\ln\left(\frac{1}{\exp(\beta)+ (k-1)\exp(-\beta)}\right)
\end{align*}

for all $i\in[2,n+1]$ and $a\in T_r$.


Note that $|T_1|=k^n$ and $|T_r^n| = k^n$,
therefore for each $t_1 \in T_1$,
we can identify a unique $t_{-1} \in T_r^n$.
More formally we consider a bijective function $c: T_1 \rightarrow T_r^n$.


We define pair-wise potentials
between the first item and the $j$-th item:
%$\psi_{i,j}(\cdot, \cdot)$ between item $i$ and item $j$:

\begin{align*}
    \psi_{1,j}(t_1,t_j) =
    \begin{cases}
    \beta  &\text{if $t_j =c(t_1)_j$} \\
    -\beta  &\text{if $t_j \neq c(t_1)_j$} \\
    \end{cases}
\end{align*}

%\begin{align*}
%    \psi_{0,j}(t_0,t_j) =
%    \begin{cases}
%    0 \quad & \text{if $i,j \neq 0$} \\
%    \beta  &\text{if $i = 0$ and $t_j =c(t_i)_j$} \\
%    -\beta  &\text{if $i = 0$ and $t_j \neq c(t_i)_j$} \\
%    \end{cases}
%\end{align*}

{Let $Z$ be the normalizing constant so that the MRF with the potentials $\{\psi_i\}_{i \in[n+1]},\{\psi_{1,i}\}_{2 \leq i \leq n+1}$ mentioned above is a valid distribution.
That is $Z = \sum_{t \in \supp(D)} \prod_{i \in [n+1]}\exp(\psi_i(t_i)) \prod_{2 \leq i \leq n+1} \exp(\psi_{1,i}(t_1,t_i))$.}
For any $t_1 \in T_1$ we have that:

\begin{align*}
    \Pr_{t'\sim D}\left[t_1' = t_1 \land t_{-1}'= c(t_1) \right] = 
    &\frac{1}{Z}\exp(\psi_1(t_1)) \frac{\exp{(n \beta)}}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \\
\end{align*}
\begin{align*}
    &\Pr_{t'\sim D}\left[t_1' = t_1 \land t_{-1}' \neq c(t_1) \right] \\ =
    &\frac{1}{Z}\exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{\substack{t_{-1} \in T_{-1}:\\ t_{-1} \neq c(t_1)}} \prod_{i \in [2,n+1]} \exp\left(\psi_{1,i}(t_1, \{t_{-1}\}_i)\right) \\
    = & \frac{1}{Z}\exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{i \in [1,n]} {n \choose i} \left(k-1 \right)^i\left(\exp(-\beta) \right)^i \left(\exp(\beta)\right)^{n-i} \\
    = & \frac{1}{Z} \exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{i \in [1,n]} {n \choose i} \left((k-1 )\exp(-\beta) \right)^i \left(\exp(\beta)\right)^{n-i} \\
    = & \frac{1}{Z} \exp(\psi_1(t_1)) \frac{(\exp(\beta)+(k-1)\exp(-\beta))^n - \exp(n \beta)}{(\exp(\beta)+(k-1)\exp(-\beta))^n} 
\end{align*}

Thus for any $t_1 \in T_1$, the marginal probability:

\begin{align*}
    f_1(t_1) = \frac{1}{Z} \exp(\psi_1 (t_1))
\end{align*}

{Note that $Z = \sum_{t_1 \in T_1} \exp(\psi_1(t_1)) = \sum_{i=0}^{k^n-2}\frac{1}{2^{i+1}} + \frac{1}{2^{k^n-1}}= 1$. Thus $f_1(t_1) = \exp(\psi_1(t_1))$.}
Therefore the marginal distribution of the first item is an Equal Revenue Distribution, which means that the revenue of any posted price mechanism for the first item, cannot be more than $1$.
Moreover, if we set $\max_{t_r \in T_r} \leq \frac{1}{2n}$,
then any posted price mechanisms for the rest $n$ items has revenue less or equal than $\frac{1}{2}$.
Thus $\srev < 2$.



Now we consider the following Mechanism in the copies settings.
We first collect the values for all the items but the first $\vT_{-1}$.
Then we let the first buyer to decide if she wants to buy the item at price $c^{-1}(t_{-1})$. This is similar to Ronen's lookahead auction~\cite{Ronen_2001}.
A lower bound on the revenue of this mechanism in the COPIES settings is:

\begin{align*}
    \sum_{t_1 \in T_1} t_1 \Pr_{t' \sim D} \left[ c^{-1}(t_{-1}) = t_1 \land t_1' =t_1 \right]
    = & \sum_{t_1 \in T_1} t_1 \exp(\psi_1(t_1)) \frac{\exp{(n \beta)}}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \\
    = & \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n\sum_{t_1 \in T_1} t_1 \exp(\psi_1(t_1))  \\
    \geq & \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n\sum_{t_1 \in T_1}\frac{1}{2}  \\
    = & \frac{1}{2} \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n|T_1| \\
    = & \frac{1}{2} \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n k^n \\
    = & \frac{1}{2} \left(\frac{k}{1 + (k-1)\exp(-2\beta)} \right)^n 
\end{align*}


Where the last inequality comes from $t_1\cdot \exp(\psi_1(t_1))  \geq \frac{1}{2}$.

Note that if we fix $\beta$ and let $k \rightarrow \infty$,
then $\lim_{k\rightarrow \infty}\left(\frac{k}{1 +(k-1)\exp(-2\beta)}\right)^n= \exp(2\beta n)$.

Therefore as $k\rightarrow \infty$,
the lower bound of the revenue of the proposed mechanisms becomes $\frac{\exp(2\beta n)}{2}$.
{Since we assumed that the value of the agent for each item except the first is less or equal than $\frac{1}{2n}$,
then the value of the agent for all but the first item is less or equal than $\frac{1}{2}$.
This implies that if the agent buys the whole bundle at price $p$,
then she also buys the first item at price $p-\frac{1}{2}$.
Let $\rev_1$ be the revenue of the posted price mechanism on the first item.
Since the marginal of the fist item is the Equal Revenue Distribution,
then $\rev_1\leq 1$.
Moreover by the argument described above,
we have that $\brev \leq \rev_1 + \frac{1}{2} < 2$.
Thus $\max(\srev, \brev) < 2$}.
\end{prevproof}










==> MRF/MRF_XOS_old.tex <==
\section{ Simple Mechanisms for an XOS Buyer }\label{sec:MRF XOS}

\subsection{Duality Framework for XOS Valuations}\label{sec:duality for XOS}

The benchmark is obtained using essentially the same approach as in \cite{CaiZ17}. Suppose the buyer has an XOS valuation function $v(\bm{t},S)$.
We denote by $V_i(\bm{t}) = v(\bm{t}, \{i\}) $.
We abuse this notation and we also define for $t_i \in T_i$,
$V_i(t_i) = v((0,\ldots,t_i,\ldots,0),\{i\}) $. We summarize the benchmark for an XOS buyer in the following Lemma. More details can be found in Appendix~\ref{sec:appx_XOS_duality}.

%\begin{definition}[Partition of Type Space for XOS valuations (similar to the type space defined in \cite{CaiZ16_arxiv})]
%We partition the type space $T$ into $n$ regions, where
%\begin{align*}
 %R_i = \{ \bm{t} \in T : \text{$f(\bm{t}) >0$ and $i$ is the smallest index that belongs in $\argmax_{i\in [n]}V_i(\vT)$  }\}   
%\end{align*}
%\end{definition}

\begin{lemma}
\label{lemma:benchmark_XOS}
Partition the type space $T$ into $n$ regions,
where
\vspace{-.1in}
\begin{align*}
 R_i = \{ \bm{t} \in T : \text{$f(\bm{t}) >0$ and $i$ is the smallest index that belongs in $\argmax_{i\in [n]}V_i(\vT)$  }\} \end{align*}
Let $r=\srev$ be the revenue of the optimal posted price mechanism that allows the buyer to purchase at most one item.
Let $C(\bm{t}) = \{ i : V_i(\bm{t}) < 2 r \}$. For any IC Mechanism $M$, we can bound its revenue by:


	\begin{align*}
\rev(M,v, D)\leq &
2\sum_{\bm{t}\in T}f(\bm{t}) \sum_{i\in [n]}  \pi_i(\bm{t})\phi(V_i(t_i) \mid \bm{t}_{-i})\mathds{1}[t \in R_i] \quad (\single)\\
%
%
&\qquad\qquad + 4\sum_{i \in [n]} \sum_{\substack{t_i \in T_i \\ V(t_i) \geq 2r}} f(t_{i}) \cdot  V_i(t_i) \Pr_{\bm{t}'\sim D}\left[\bm{t}'\notin R_i \mid t_i'=t_i \right](\tail) \\
%
%
 & \qquad\qquad\qquad\qquad+  4\sum_{\bm{t}\in T}f(\bm{t}) v(\vT,C(\bm{t}))\quad(\core)
 	\end{align*}
 	
\end{lemma}




\subsection{Approximating the Benchmark of an XOS Buyer}
In this section, we show how to approximate the optimal revenue of a buyer with an XOS valuation. We first upper bound the term \single~  and \tail~. The analysis of both terms follows from the combination of the analysis in~\cite{CaiZ17} and Lemma~\ref{lemma:tv_MRF}.
\begin{lemma}\label{lemma:XOS_single_tail}
Let the type distribution $D$ be a MRF and $M$ be an IC mechanism for a buyer with an XOS valuation. The following inequalities holds $\single \leq 4\exp(12\Delta(\bm{t}))\cdot \srev$ and $\tail \leq \exp(8\Delta(\bm{t})) \cdot \srev $, where $\srev$ is the revenue of the optimal posted price auction, in which the buyer is allowed to purchase at most one item.

\end{lemma}





%In the following subsection we provide the necessary techniques that we need in order to bound the $(\core)$.

\subsubsection{Bounding the \core~using the Poincar\'{e} Inequality}\label{sec:XOS_core}

In this section, we show how to bound the \core~for an XOS buyer. The $\core$ is the expectation of the random variable $v(\vT,C(\vT))$. To show that bundling can achieve a good approximation of the \core, we need to upper bound the variance of $v(\vT,C(\vT))$. This is the main technical task for this section. As $v(\vT,\cdot)$ is not additive across the items, our method for the additive valuation (see Lemma~\ref{lemma:cov}) no longer applies. We provide a new approach that is based on the \emph{Poincar\'{e} Inequality}~\cite{wu2006} and the \emph{self-boundingness of XOS functions}. We first provide the necessary notation and techniques.


\begin{definition}[Self-Bounding Functions~\cite{BoucheronLM00}]\label{def:self-bounding}
We say that a function $g(\vT): \mathbb{E}^n \rightarrow \mathbb{R}$,
where $\E$ can be any set,
is \emph{$C$-self-bounding} with some constant $C\in \mathbb{R}_+$ if there exists functions $g_i:\E^{n-1}\rightarrow \mathbb{R}$ for all $i\in[n]$ such that for each $\vT \in \E^n$ the followings hold:
\begin{itemize}
    \item $0 \leq g(\vT)-g_i(\vT_{-i}) \leq C$ for all $i\in[n]$.
    \item $\sum_{i\in[n]} \left(g(\vT)-g_i(\vT_{-i})\right)\leq g(\vT)$. 
\end{itemize}


\end{definition}



\noindent Next, we show that $g(\vT)=v(\vT,C(\vT))$ is $2\srev$-self-bounding. The proof is postponed to Appendix~\ref{sec:appx_XOS_single_tail}. Recall that $C(\bm{t}) = \{ j : V_j(\bm{t}) < 2 \srev\}$.

\begin{lemma}
\label{lemma:self_bounding_MRF}
The function $g(\vT)=v(\vT,C(\vT))$ is $2\srev$-self-bounding.
\end{lemma}




%Now we are going to provide a Theorem from \cite{wu2006} that helps us bound the $(\core)$.
To state the Poincar\'{e} Inequality, we first introduce the notion of \emph{Dobrushin's Interdependence Matrix}.

\begin{definition}[$d$-Dobrushin Interdependence Matrix~\cite{wu2006}]\label{def:Dobrushin's interdependence matrix}
Let $(\E,d)$ be a metrical, complete and separable space.
For two distributions $\mu$ and $\nu$ supported on $\E$,
their $L^1$-Wasserstein distance is defined as:    $$W_{1,d}(\mu,\nu) = \inf_{\pi \in \Pi} \int\int_{\E \times \E} d(x,y) \pi(dx,dy),$$ where $\Pi$ is the set of valid coupling such that its marginal distributions are $\mu$ and $\nu$.


Let $X=(x_1,\ldots, x_n)$ be a $n$-dimensional random vector supported on $\E^n$ and $\mu_i(\cdot \mid x_{-i})$ be the conditional distribution of $x_i$ knowing $x_{-i}$. 
Define the \textbf{$d$-Dobrushin Interdependence Matrix} $A=(\alpha_{i,j})_{i,j\in[n]}$ by
$$\alpha_{i,j}:= \sup_{\substack{x_{-i-j}=y_{-i-j}\\ x_j\neq y_j}}\frac{W_{1,d}(\mu_i(\cdot\mid x_{-i}),\mu_i(\cdot\mid y_{-i}))}{d(x_j,y_j)}.$$

\paragraph{Dobrushin uniqueness condition:} If we choose $d(x,y)$ to be the trivial metric $\ind_{x\neq y}$, then $W_{1,d}(\cdot,\cdot)$ is exactly the total variation distance. Under the trivial metric, we define the \textbf{Dobrushin Coefficient} as $\alpha(\vT):=||A||_\infty=\max_{i\in [n]} \sum_{j\neq i} \alpha_{i,j}$. If $\alpha(\vT)<1$, we  say $\vT$ satisfies the \textbf{Dobrushin uniqueness condition}.
\end{definition}
\begin{remark}
$\alpha_{i,j}$ captures how strong the value of $x_j$ affects the conditional distribution of
$x_i$ when all other coordinates are fixed. Higher $\alpha_{i,j}$ value implies stronger dependence between $x_i$ and $x_j$. When all the coordinates of $X$ are independent, $A$ is the all zero matrix. %The \textbf{Dobrushin uniqueness condition} was originally introduced by Dobrushin~\cite{Dobruschin68} in the study of Gibbs measures, in the context of identifying conditions under which the Gibbs distribution has a unique equilibrium. Since then, the model has been extensively studied in statistical physics and probability literature (see e.g.~\cite{DobrushinS87,StroockZ92}). The condition has recently been used to model weakly dependent random variables~\cite{DaganDDJ19}.%The Dobrushin uniqueness condition can also be %implies a number of desirable properties, such as fast mixing of Glauber dynamics~\cite{Kulske03}, concentration of measure~\cite{Chatterjee05, Daskalakis18,Gheissari18,Kulske03,Marton96}, and correlation decay~\cite{Kunsch82}, and has been used as . For a survey of properties resulting from Dobrushin's condition see~\cite{Weitz05}.
\end{remark}
Now we are ready to present the Poincar\'e inequality. %Very high-levelly speaking,
At a high level,
Poincar\'{e} inequalities connect the variance of a function $g(\cdot)$ with the $\ell_2$-norm of the gradient of $g(\cdot)$, and usually take the form of $\Var_{X\sim D}[g(X)]\lesssim\E_{X\sim D}[||\text{gradient}(g(X))||^2]$. These inequalities are called \emph{Poincar\'e inequalities} because Poincar\'{e} first published an inequality of this type for the uniform distribution on a bounded domain in $\mathbb{R}^n$, ca. 1890. Many similar inequalities have since been discovered. One notable example is the Efron-Stein inequality~\cite{efron1981jackknife}, which has numerous applications in combinatorics, statistics, and statistical learning~\cite{massart2007concentration,boucheron2013concentration}. The Efron-Stein inequality only applies to \emph{independent random variables}. The following result by Wu~\cite{wu2006} provides a generalization of the Efron-Stein inequality for \emph{weakly dependent random variables}.

\begin{lemma}[Poincar\'{e} Inequality for Weakly Dependent Random Variables \cite{wu2006}]
\label{thm:var_d}
Let $\vT=(t_1,\ldots,t_n)$ be an $n$-dimensional random vector drawn from distribution $D$ that is supported on $\E^n$. For any metric $d(\cdot,\cdot)$ on $\E$, let $A$ be the $d$-Dobrushin interdependence matrix for $\vT$. Let $\rho_d(\vT)$ be the spectral radius of $A$ (which is the dominant eigenvalue of $A$ by the Perron-Frobenius Theorem).
If $\E_{\vT \sim D}\left[ \sum_{i\in[n]} d(t_i,y_i)^2 \right] < + \infty$ for some fixed $y \in \E^n$ and  $\rho_d(\vT) < 1$, then for any square integrable function $g(\cdot)$ w.r.t. distribution $D$, the following holds:
$$    (1-\rho_d(\vT))\Var_{\vT\sim D}[g(\vT)] \leq \sum_{i \in [n]} \E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( f(t_i,\vT_{-i}) - \E_{t_i \sim D_{i \mid \vT_{-i}}}[f(t_i,\vT_{-i})] \right)^2 \right] \right].$$
\end{lemma}

\begin{remark}
In the independent case, $\rho_d(\vT)=0$, which recovers the Efron-Stein inequality. The condition that $\rho_d(\vT)<1$ is a natural condition. Firstly, it is implied by the \textbf{Dobrushin uniqueness condition} (see Section~\ref{subsec:core_dob} for more discussion). Secondly, the condition implies rapid mixing of the Glauber dynamics (see Lemma~\ref{lemma:rapid mixing}). A special case of Lemma~\ref{lemma:rapid mixing}, where $d(x,y)=\ind_{x\neq y}$, was shown by Hayes~\cite{Hayes06}. %We provide the general case here for completeness. %related to the $d$-Dobrushin interdependence matrix is the \textbf{Dobrushin uniqueness condition}, which was originally introduced by Dobrushin~\cite{Dobruschin68} in the study of Gibbs measures, in the context of identifying conditions under which the Gibbs distribution has a unique equilibrium. Since then, the model has been extensively studied in statistical physics and probability literature (see e.g.~\cite{DobrushinS87,StroockZ92}). The Dobrushin uniqueness condition can also be %implies a number of desirable properties, such as fast mixing of Glauber dynamics~\cite{Kulske03}, concentration of measure~\cite{Chatterjee05, Daskalakis18,Gheissari18,Kulske03,Marton96}, and correlation decay~\cite{Kunsch82}, and has been used as . For a survey of properties resulting from Dobrushin's condition see~\cite{Weitz05}. We plan to investigate the following question.

\end{remark} 

\argyrisnote{
From now on,
we may use character $d$ to denote a metric on a space,
or the weighted degree of the $i$-th item on a MRF $d_i(\cdot)$.
We are going to omit what character $d$ refers to
when it is clear from the context.
}


Although the RHS of the Poincar\'{e} inequality may seem complicated, we show that it can be  upper bounded by $O(\E[g(\vT)])$ when $g(\cdot)$ is a self-bounding function.
\begin{lemma} \label{lemma:sum_bound}
Let $g$ be a $C$-self-bounding function.
Then:
\begin{align*}
    \sum_{i \in [n]} \E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - \E_{t'_i \sim D_{i \mid \vT_{-i}}}[g(t'_i,\vT_{-i})] \right)^2 \right] \right] \leq C \E_{\vT \sim D} \left[ g(\vT) \right]
\end{align*}
\end{lemma}

\begin{proof}
 Recall the following property of the variance: for any real-value random variable $X$, $\Var[X]=\min_{a\in R} \E[(X-a)^2]$. In other words, $\Var[X]\leq \E[(X-a)^2]$ for any $a$. Therefore, for any $\vT_{-i}$, $$\E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - \E_{t'_i \sim D_{i \mid \vT_{-i}}}[g(t'_i,\vT_{-i})] \right)^2\right] = \Var[g(\vT)\mid \vT_{-i}]\leq \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - g_i(\vT_{-i}) \right)^2\right].$$ 
 
Using this relaxation, we proceed to prove the claim.
\begin{align*}
    & \sum_{i \in [n]}\E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid t_{-i}}} \left[ \left( f(t_i,t_{-i}) - \E_{t_i \sim D_{i \mid t_{-i}}}[f(t_i,t_{-i})] \right)^2 \right] \right]\\
    \leq & \sum_{i \in [n]}\E_{\vT \sim D} \left[ \left( g(\vT) - g_i(\vT_{-i}) \right)^2 \right]
    \leq  C \sum_{i \in [n]}\E_{\vT \sim D} \left[ \left(g(\vT) - g_i(\vT_{-i})\right) \right]
    \leq  C \E_{\vT \sim D} \left[ g(\vT) \right]
\end{align*}

\end{proof}
\notshow{
Therefore,
if we want to bound the variance of  $v(\vT,C(\vT))$,
when its input is sampled from a MRF $D$,
it is enough to define a metric $d$,
such that the infinite norm of the $d$-Dobrushin interdependence matrix of $D$ (as defined in Theorem~\ref{thm:var_d}) is less than $1$.


The goal of the following subsections is to use the flexibility that Theorem~\ref{thm:var_d} provides us to define a metric $d$  so that we can derive meaningful bounds for the variance of $v(\vT,C(\vT))$.

\subsubsection{Putting Everything Together}


We can unify the bounds derived in Subsection~\ref{subsec:core_dob}, Subsection~\ref{subsec:core_trees} and Subsection~\ref{subsec:core_d_trees} for the variance of $v(\vT, C(\vT))$ by considering a variable $c\in [0,1\}$ (that depends on the MRF $D$ that we consider) such that $Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1 - c}$.

}

Now, we show how to approximate $\core$ using $\srev$ and $\brev$.

\begin{lemma}\label{lemma:XOS_core}
%Let $D$ be a MRF such that $Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1- c}$,
Let $d(\cdot,\cdot)$ be a metric and $\rho_d(\vT)$ be  the spectral radius of the $d$-Dobrushin interdependence matrix of $\vT$. If $\rho_d(\vT)\in[0,1)$, then $\Var[v(\vT,C(\vT))] \leq \frac{2\srev\cdot \core}{1 - \rho_d(\vT)}$. Moreover,
$$\core \leq \max\left( \frac{4\srev}{\sqrt{1-\rho_d(\vT)}} ,\left(7 + \frac{4}{\sqrt{1-\rho_d(\vT)}} \right)\brev \right).$$
\end{lemma}
\begin{proof}
According to Lemma~\ref{lemma:self_bounding_MRF}, $v(\vT,C(\vT))$ is a $2\srev$-self-bounding function. Combining Lemma~\ref{thm:var_d} and Lemma~\ref{lemma:sum_bound}, we can further show that $\Var[v(\vT,C(\vT)]\leq \frac{2\srev\cdot \E_{\vT\sim D}[v(\vT,C(\vT)]}{1-\rho_d(\vT)}=\frac{2\srev\cdot \core}{1-\rho_d(\vT)}$.

If $\core \leq \frac{4\srev}{\sqrt{1-\rho_d(\vT)}}$,
then the statement holds. If $\core > \frac{4\srev}{\sqrt{1-\rho_d(\vT)}}$,
then $\Var[v(\vT,C(\vT))] \leq \frac{2\core\cdot \srev}{1-\rho_d(\vT)} <  \frac{(\core)^2}{2\sqrt{1-\rho_d(\vT)}} = \frac{ \E[v(\vT,C(\vT))]^2}{2\sqrt{1-\rho_d(\vT)}}$.
By Paley-Zygmund inequality we have that:
    $$ \Pr\left[ v(\bm{t},C(\bm{t})) \geq \frac{\core}{3}  \right] 
    \geq \frac{4}{9} \frac{1}{1 + \frac{\Var[v(\vT,C(\vT))]}{\E[v(\vT,C(\vT))]^2}} 
    \geq  \frac{4}{9} \frac{1}{1 + \frac{1}{2\sqrt{1-\rho_d(\vT)}}} .$$
Therefore we have that: $\Pr\left[ v(\bm{t},C(\bm{t})) \geq \frac{\core}{3}  \right]\cdot \frac{\core}{3} \leq \brev$, which implies that the statement. %$$ \core \leq \frac{27}{4}\left(1 + \frac{1}{2\sqrt{1-\rho_d(\vT)}}\right)\brev \leq \left(7 + \frac{4}{\sqrt{1-\rho_d(\vT)}}\right) \brev.$$

\end{proof}

Finally, we combine our analysis of \single, \tail, and \core~to obtain the approximation guarantee for an XOS buyer.
\begin{theorem}\label{thm:XOS}
 Let the XOS buyer's type $\vT$ be generated by a MRF $D$. If there exists metric $d(\cdot,\cdot)$ such that $\rho_d(\vT)\in[0,1)$, then the revenue obtained by any IC mechanism $M$ is bounded by: 
    $$\rev(M,v, D)\leq  12\exp(12\Delta(\vT)) \cdot \srev + \left(28 + \frac{16}{\sqrt{1-\rho_d(\vT)}}\right)\max\{\srev,\brev\}.$$ 
\end{theorem}
\begin{prevproof}{Theorem}{thm:XOS}
The statement follows from the combination of Lemma~\ref{lemma:XOS_single_tail} and Lemma~\ref{lemma:XOS_core}.
\end{prevproof}

\paragraph{Inapproximability under the Dobrushin uniqueness condition} Readers may wonder whether it is possible to prove an approximation ratio that only relies on either the spectral radius $\rho_d(\vT)$ or the Dobrushin coefficient $\alpha(\vT)$, but not the maximum weighted degree $\Delta(\vT)$. We show that this is impossible. Indeed, we prove that for any $\alpha<1$, and any ratio $N$, there exists an MRF with $\rho_d(\vT)\leq\alpha(\vT)\leq\alpha$ such that the ratio between the optimal revenue and $\max\{\brev(D),\srev(D)\}$ is at least $\frac{\alpha}{2}\cdot N$. Our result is based on a modification of the Hart-Nisan construction~\cite{HARTN_2019} and can be found in Appendix~\ref{sec:inapprox_Dobrushin}.
\begin{theorem}\label{lem:inaprx_dob}
For any positive real number $N$ and any choice of $0< \alpha \leq 1$,
there exists a type distribution over $2$ items generated by a MRF $D$ with $\alpha(\vT) = \alpha$ and finite inverse temperature,
such that for an additive buyer whose type is sampled from $D$,
$\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}>\frac{\alpha}{2}\cdot N$.
\end{theorem}

\paragraph{High Temperature MRFs.}\label{subsec:core_dob}
We consider the case where the buyer type $\vT$ is \emph{high temperature}, i.e., $\beta(\vT) < 1$ (see Definition~\ref{def:Markov influence}). We show that for any XOS valuation and constant inverse temperature $\beta(\vT)<1$, $\max\{\srev,\brev\}$ is a constant factor approximation to the optimal revenue. By the definition of $\beta(\vT)$, it clear that $\Delta(\vT)\leq \beta(\vT)$. Next, we show that $\beta(\vT)$ is also an upper bound of $\rho_d(\vT)$ for the trivial metric $d(x,y)=\ind_{x\neq y}$. Due to limited space, the proof is delayed to Appendix~\ref{sec:appx_special_cases}.

\begin{lemma}\label{lemma:Dobruthin properties}
Let $d(\cdot,\cdot)$ be the trivial metric $d(x,y)=\ind_{x\neq y}$. For any MRF $\vT$, $\rho_d(\vT)\leq \alpha(\vT)\leq \beta(\vT)$. Moreover, $\alpha_{i,j}\leq \beta_{i,j}(\vT)$ for all $i,j\in[n]$.
\end{lemma}

\begin{theorem}\label{thm:XOS_high_temperature}

If the type of an XOS buyer $\vT$ is high temperature, i.e., $\beta(\vT)<1$,
$$\rev(v, D)\leq  12\exp(12\beta(\vT)) \cdot \srev + \left(28 + \frac{16}{\sqrt{1-\beta(\vT)}}\right)\max\{\srev,\brev\}.$$
\end{theorem}
\begin{prevproof}{Theorem}{thm:XOS_high_temperature}
The statement follows from Theorem~\ref{thm:XOS} and Lemma~\ref{lemma:Dobruthin properties}.
\end{prevproof}


%where $c = \alpha^M$ if the MRF $D$ satisfies the Dobrushin Uniqueness Condition, or $c = 2\beta \sqrt{d}$ if the MRF $D$ is over a $d$-ary tree such that the highest value of the Markov Correlation for any pair of items is bounded by $\beta < \frac{1}{2\sqrt{d}}$.



























==> MRF/appx_MRF_properties.tex <==
\section{Missing Proofs from Section~\ref{sec:basic MRF properties}}\label{sec:appx_MRF_properties}
\argyrisnote{I moved the proof of this section to the main body}

\begin{prevproof}{Lemma}{lemma:cond_MRF}
Note that for any $t_i'\in T_i$, 
${f\left((t_i,t_{-i})\right)\over f\left((t_i',t_{-i})\right)}={\exp(\psi_i(t_i))\over \exp(\psi_i(t'_i))}\cdot {\exp\left(\sum_{e\in E, i\in e} \psi_e\left( t_i, t_{-i}\right)_e\right) \over \exp\left(\sum_{e\in E, i\in e} \psi_e\left( t'_i, t_{-i}\right)_e\right) }$. 


%${f\left((t_i,t_{-i})\right)\over f\left((t_i',t_{-i})\right)}={\exp(\psi_i(t_i))\over \exp(\psi_i(t'_i))}\cdot {\exp\left(\sum_{e\in E, i\in e} \exp(\psi_e\left( t_i, t_{-i}\right)_e)\right) \over \exp\left(\sum_{e\in E, i\in e} \exp(\psi_e\left( t'_i, t_{-i}\right)_e)\right) }$. 

Clearly, $${\exp(\psi_i(t_i))\over \exp(\psi_i(t'_i))}\cdot \exp(-2\Delta(\vT))\leq {f\left((t_i,t_{-i})\right)\over f\left((t_i',t_{-i})\right)}\leq {\exp(\psi_i(t_i))\over \exp(\psi_i(t'_i))}\cdot \exp(2\Delta(\vT)).$$

Since $f_i(t_i\mid t_{-i}) = {f\left((t_i,t_{-i})\right)\over\sum_{t_i'\in T_i}f\left((t_i',t_{-i})\right)}$, $$\frac{\exp(\psi_i(t_i))\cdot\exp(-2 \Delta(\vT))}{\sum_{t'_i \in T_i} \exp(\psi_i(t_i'))} \leq f_i(t_i\mid t_{-i}) \leq \frac{\exp(\psi_i(t_i))\exp(2 \Delta(\vT))}{\sum_{t'_i \in T_i} \exp(\psi_i(t_i'))}.$$
By Law of Total Probability,
\begin{align*}
    f_i(t_i) = & \sum_{t_{-i} \in T_{-i}} f_i(t_i \mid t_{-i}) f_{-i} (t_{-i})\in\left[\frac{\exp(\psi_i(t_i))\cdot\exp(-2\Delta(\vT))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))} ,\frac{\exp(\psi_i(t_i))\cdot \exp(2\Delta(\vT))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))}\right].
\end{align*}

\end{prevproof}


\begin{prevproof}{Lemma}{lemma:tv_MRF}
%Note that $\Pr_{\vT\sim D}\left[t_i\in \EE \land t_{-i}\in \EE' \right] =\sum_{\vT\in \EE \times \EE'} f_i(t_i\mid t_{-i})\cdot f_{-i}(t_{-i})$ and  $\Pr[t_i\in \EE] \Pr\left[t_{-i}\in \EE'\right]= \sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})$. Hence, our claim follows from Lemma~\ref{lemma:cond_MRF}.
Note that $\Pr_{\vT\sim D}\left[t_i\in \EE \land t_{-i}\in \EE' \right] =\sum_{\vT\in \EE \times \EE'} f_i(t_i\mid t_{-i})\cdot f_{-i}(t_{-i})$ and  $\Pr[t_i\in \EE] \Pr\left[t_{-i}\in \EE'\right]= \sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})$.
Hence
$$
{ \Pr_{\vT\sim D}\left[t_i\in \EE \land t_{-i}\in \EE' \right] \over \Pr_{t_i\sim D_i}[t_i\in \EE] \Pr_{t_{-i}\sim D_{-i}}\left[t_{-i}\in \EE'\right]}  = \frac{\sum_{\vT\in \EE \times \EE'} f_i(t_i\mid t_{-i})\cdot f_{-i}(t_{-i})}{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})}
$$
Using Lemma~\ref{lemma:cond_MRF} we get that:
$$
 \frac{\sum_{\vT\in \EE \times \EE'} f_i(t_i\mid t_{-i})\cdot f_{-i}(t_{-i})}{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})} \leq \exp(4\Delta) \frac{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})}{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})} = \exp(4\Delta)
$$
and
$$
 \frac{\sum_{\vT\in \EE \times \EE'} f_i(t_i\mid t_{-i})\cdot f_{-i}(t_{-i})}{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})} \geq \exp(-4\Delta) \frac{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})}{\sum_{\vT\in \EE \times \EE'} f_i(t_i)\cdot f_{-i}(t_{-i})} = \exp(-4\Delta).
$$

\notshow{Similarly we can prove that  $\Pr[t_i] \geq \frac{\exp(\psi_i(t_i))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))}\exp(-2\Delta)$


Noting that:

\begin{align*}
\frac{\exp(\psi_i(t_i))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))}\exp(-2\Delta) \leq \Pr[t_i] \leq \frac{\exp(\psi_i(t_i))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))}\exp(2\Delta) \\
\frac{\exp(\psi_i(t_i))}{\sum_{t_i' \in T_i} \exp(\psi_i(t_i'))}\exp(-2\Delta) \leq \Pr[t_i=t\mid t_{-i}] \leq \frac{\exp(\psi_i(t_i))}{\sum_{t_i'\in T_i} \exp(\psi_i(t_i'))}\exp(2\Delta)
\end{align*}

We can infer that:

\begin{align*}
\Pr[t_i] \exp(-4\Delta) \leq \Pr[t_i\mid t_{-i}] \leq \Pr[t_i] \exp(4\Delta)
\end{align*}

Therefore we have that:

\begin{align*}
    \Pr[t > t_i \mid t_{-i}] =  \sum_{t_i' > t_i} \Pr[t_i' \mid t_{-i}] \leq \sum_{t_i' > t_i} \Pr[t_i'] \exp(4\Delta) = \Pr[t > t_i] \exp(4\Delta)
\end{align*}

We can similarly prove that $\Pr[t > t_i\mid t_{-i}] \geq \Pr[t > t_i] \exp(-4\Delta) $
}
\end{prevproof}

\begin{prevproof}{Lemma}{lemma:MRF_prophet}
The proof is similar to the case when all $t_i$ are independent.

It is not hard to see that $$\E_{\vT}\left[\max_{i\in [n] }g_i(t_i)\right]\leq \tau^*+\sum_{i\in [n]} \E_{t_i\sim D_i}\left[\left(g_i(t_i)-\tau^*\right)^+\right].$$

We provide a lower bound on $\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]$.
\begin{align*}
	\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]\geq \Pr_{\vT}\left[\max_{i\in[n]} g_i (t_i)  \geq \tau^*\right] \cdot \tau^* + \sum_{i\in [n]}\E_{\vT}\left[(g_i(t_i) - \tau^*)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) \leq \tau^*] \right]
\end{align*}  
For every $i\in [n]$, we define the set $\EE_{i}$ as $\{t_i\in T_i : g_i(t_i)> \tau^*\}$ and $\EE'_{i}$ as $\{t_{-i}\in T_{-i}: \max_{j\neq i} g_j(t_j)\leq\tau^* \}$. Note that 
\begin{align*}
\E_{\vT}\left[(g_i(t_i) - \tau^*)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau^*] \right]
&=\sum_{\vT\in \EE_i\times \EE_i'}\left(g_i(t_i)-\tau^*\right)\cdot f(\vT)\\	
&\geq \exp(-4\Delta(\vT)) \sum_{\vT\in \EE_i\times \EE_i'}\left(g_i(t_i)-\tau^*\right)\cdot f_i(t_i)f_{-i}(t_{-i})\\
&= \exp(-4\Delta(\vT))\E_{t_i\sim D_i}\left[\left(g_i(t_i)-\tau^*\right)^+\right]\Pr_{t_{-i}\sim D_{-i}}[t_{-i}\in \EE'_i]
\end{align*}

The inequality is due to Lemma~\ref{lemma:tv_MRF}. Putting everything together, we know that 
$$\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]\geq {1\over 2} \cdot \tau^* + \sum_{i\in [n]}\E_{t_i\sim D_i}\left[(g_i(t_i) - \tau^*)^+\right]\cdot {\exp(-4\Delta(\vT))\over 2},
$$ which is at least ${\exp(-4\Delta(\vT))\over 2}$ of the upper bound we provide for $\E_{\vT}\left[\max_{i\in [n] }g_i(t_i)\right]$.
\footnote{When $\max_{i \in [n]}g_i(t_i)$ is a discrete distribution, we may not be able to pick a $\tau^*$ such that $\Pr[\max_{i \in [n]}g_i(t_i) \geq \tau^*]=1/2$, but it is folklore that this can be resolved by carefully picking a tie-breaking rule. We do not include the details here.}
%
%\argyrisnote{(I think the next sentence should not be here)}
%The proof is similar for $\tau^*=\min_{\tau}\left\{\tau\in \mathbb{R}: \Pr_{\vT}\left[\max_{i\in [n]} g_i(t_i)\leq \tau\right]\geq {\exp(4\Delta(\vT))\over 1+\exp(4\Delta(\vT))}\right\}$.
%\todo{Say something about tie breaking}
\notshow{
Fix an item $i$.
\begin{comment}
We can write

\begin{align*}
Pr[t_i \cap \max_{j \neq i} t_j < \tau] = \sum_{\substack{t_{-i} \in T_{-i}: \\ \max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i \mid t_{-i}] \cdot Pr[t_{-i}] 
\end{align*}

By Lemma~\ref{lemma:cond_MRF} we have that:

\begin{align*}
\sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i \mid t_{-i}] \cdot Pr[t_{-i}] 
\geq & \sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i] \exp(-2\Delta) \cdot Pr[t_{-i}]  \\
= & Pr[t_i] \exp(-2\Delta) \sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_{-i}]  \\
= & Pr[t_i] \exp(-2\Delta) Pr[\max_{j\neq i} \varphi_j(t_j) < \tau] 
\end{align*}

This implies that:

\begin{align*}
    Pr[t_i \cap \max_{j \neq i} t_j < \tau] \geq Pr[t_i] \exp(-2\Delta) Pr[\max_{j\neq i} \varphi_j(t_j) < \tau] 
\end{align*}

\end{comment}

Using Lemma~\ref{lemma:tv_MRF} with condition function $C(T_{-i})=\mathds{1}[\max_{j\neq i} g_j(t_j) < \tau]$ we have that:

\begin{align*}
    \Pr[t_i \cap \max_{j \neq i} t_j < \tau] \geq \Pr[t_i] \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] 
\end{align*}


An upper bound on $E[\max_i g(t_i)]$ is:

\begin{align*}
    \tau + \sum_{i}E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}





A lower bound on the prophet reward is:

\begin{align*}
    &\Pr[\max_i g_i (x_i) \geq \tau] \cdot \tau + E\left[\sum_{i}(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right] \\
    = & \Pr[\max_i g_i (t_i) \geq \tau] \cdot \tau + \sum_{i}E\left[(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right]
\end{align*}

We have that:

\begin{align*}
    &E \left[(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right] \\
    = & \sum_{\substack{t_i \in T_i: \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \cap  \max_{j \neq i} t_j < \tau \right] \\
    \geq & \sum_{\substack{t_i \in T_i \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \right] \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \\
    = & \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \cdot \sum_{\substack{t_i \in T_i \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \right] \\
    = & \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}

Therefore a lower bound on the prophet's reward is:

\begin{align*}
    &\tau \cdot \Pr[\max_{i} g_i(t_i) \geq \tau] + \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \sum_i E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}

By choosing a value of $\tau$ such that $\Pr[\max_i g_i(x_i) \geq \tau] = \frac{1}{2}$,
then we also have that for any $i$: $\Pr[\max_{j\neq i} g_j(x_j)< \tau] \geq \Pr[\max_{j} g_j(x_j)< \tau] = \frac{1}{2}$.

The lower bound on Prophet's reward is:

\begin{align*}
\frac{1}{2} \tau + \frac{\exp(-2\Delta)}{2}\sum_i E \left[ (g_i(t_i) - \tau)^+ \right] \geq 
\frac{\exp(-2\Delta)}{2}\left( \tau + \sum_i E \left[ (g_i(t_i) - \tau)^+ \right]\right) 
\end{align*}

And the statement is proved.

}
\end{prevproof}



\notshow{
\argyrisnote{
\begin{prevproof}{Lemma}{lemma:MRF_prophet}
The proof is similar to the case when all $t_i$ are independent.

It is not hard to see that $$\E_{\vT}\left[\max_{i\in [n] }g_i(t_i)\right]\leq \tau^*+\sum_{i\in [n]} \E_{t_i\sim D_i}\left[\left(g_i(t_i)-\tau^*\right)^+\right].$$

We provide a lower bound on $\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]$.
\begin{align*}
	\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]\geq \Pr_{\vT}\left[\max_{i\in[n]} g_i (t_i)  \geq \tau^*\right] \cdot \tau^* + \sum_{i\in [n]}\E_{\vT}\left[(g_i(t_i) - \tau^*)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau^*] \right]
\end{align*}  
For every $i\in [n]$, we define the set $\EE_{i}$ as $\{t_i\in T_i : g_i(t_i)\geq \tau^*\}$ and $\EE'_{i}$ as $\{t_{-i}\in T_{-i}: \max_{j\neq i} g_j(t_j) < \tau^* \}$. Note that 
\begin{align*}
\E_{\vT}\left[(g_i(t_i) - \tau^*)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau^*] \right]
&=\sum_{\vT\in \EE_i\times \EE_i'}\left(g_i(t_i)-\tau^*\right)\cdot f(\vT)\\	
&\geq \exp(-4\Delta(\vT)) \sum_{\vT\in \EE_i\times \EE_i'}\left(g_i(t_i)-\tau^*\right)\cdot f_i(t_i)f_{-i}(t_{-i})\\
&= \exp(-4\Delta(\vT))\E_{t_i\sim D_i}\left[\left(g_i(t_i)-\tau^*\right)^+\right]\Pr_{t_{-i}\sim D_{-i}}[t_{-i}\in \EE'_i]
\end{align*}

The inequality is due to Lemma~\ref{lemma:tv_MRF}. Putting everything together, we know that 
$$\rew_{\vT}\left[\{g_i\}_{i\in [n]}, \tau^*\right]\geq {1\over 2} \cdot \tau^* + \sum_{i\in [n]}\E_{t_i\sim D_i}\left[(g_i(t_i) - \tau^*)^+\right]\cdot {\exp(-4\Delta(\vT))\over 2},
$$ which is at least ${\exp(-4\Delta(\vT))\over 2}$ of the upper bound we provide for $\E_{\vT}\left[\max_{i\in [n] }g_i(t_i)\right]$.


\argyrisnote{(I think the following sentence was not meant to be there)}


The proof is similar for $\tau^*=\min_{\tau}\left\{\tau\in \mathbb{R}: \Pr_{\vT}\left[\max_{i\in [n]} g_i(t_i)\leq \tau\right]\geq {\exp(4\Delta(\vT))\over 1+\exp(4\Delta(\vT))}\right\}$.
%\todo{Say something about tie breaking}
\notshow{
Fix an item $i$.
\begin{comment}
We can write

\begin{align*}
Pr[t_i \cap \max_{j \neq i} t_j < \tau] = \sum_{\substack{t_{-i} \in T_{-i}: \\ \max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i \mid t_{-i}] \cdot Pr[t_{-i}] 
\end{align*}

By Lemma~\ref{lemma:cond_MRF} we have that:

\begin{align*}
\sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i \mid t_{-i}] \cdot Pr[t_{-i}] 
\geq & \sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_i] \exp(-2\Delta) \cdot Pr[t_{-i}]  \\
= & Pr[t_i] \exp(-2\Delta) \sum_{\substack{t_{-i} \in T_{-i}: \\\max_{j \neq i} \varphi_j(t_j) < \tau}} Pr[t_{-i}]  \\
= & Pr[t_i] \exp(-2\Delta) Pr[\max_{j\neq i} \varphi_j(t_j) < \tau] 
\end{align*}

This implies that:

\begin{align*}
    Pr[t_i \cap \max_{j \neq i} t_j < \tau] \geq Pr[t_i] \exp(-2\Delta) Pr[\max_{j\neq i} \varphi_j(t_j) < \tau] 
\end{align*}

\end{comment}

Using Lemma~\ref{lemma:tv_MRF} with condition function $C(T_{-i})=\mathds{1}[\max_{j\neq i} g_j(t_j) < \tau]$ we have that:

\begin{align*}
    \Pr[t_i \cap \max_{j \neq i} t_j < \tau] \geq \Pr[t_i] \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] 
\end{align*}


An upper bound on $E[\max_i g(t_i)]$ is:

\begin{align*}
    \tau + \sum_{i}E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}





A lower bound on the prophet reward is:

\begin{align*}
    &\Pr[\max_i g_i (x_i) \geq \tau] \cdot \tau + E\left[\sum_{i}(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right] \\
    = & \Pr[\max_i g_i (t_i) \geq \tau] \cdot \tau + \sum_{i}E\left[(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right]
\end{align*}

We have that:

\begin{align*}
    &E \left[(g_i(t_i) - \tau)^+ \cdot \mathds{1}[\max_{j\neq i} g_j(t_j) < \tau] \right] \\
    = & \sum_{\substack{t_i \in T_i: \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \cap  \max_{j \neq i} t_j < \tau \right] \\
    \geq & \sum_{\substack{t_i \in T_i \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \right] \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \\
    = & \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \cdot \sum_{\substack{t_i \in T_i \\ t_i \geq \tau }}  \left( g_i(t_i) - \tau\right) \Pr\left[ t_i \right] \\
    = & \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}

Therefore a lower bound on the prophet's reward is:

\begin{align*}
    &\tau \cdot \Pr[\max_{i} g_i(t_i) \geq \tau] + \exp(-2\Delta) \Pr[\max_{j\neq i} g_j(t_j) < \tau] \sum_i E \left[ (g_i(t_i) - \tau)^+ \right]
\end{align*}

By choosing a value of $\tau$ such that $\Pr[\max_i g_i(x_i) \geq \tau] = \frac{1}{2}$,
then we also have that for any $i$: $\Pr[\max_{j\neq i} g_j(x_j)< \tau] \geq \Pr[\max_{j} g_j(x_j)< \tau] = \frac{1}{2}$.

The lower bound on Prophet's reward is:

\begin{align*}
\frac{1}{2} \tau + \frac{\exp(-2\Delta)}{2}\sum_i E \left[ (g_i(t_i) - \tau)^+ \right] \geq 
\frac{\exp(-2\Delta)}{2}\left( \tau + \sum_i E \left[ (g_i(t_i) - \tau)^+ \right]\right) 
\end{align*}

And the statement is proved.

}
\end{prevproof}
}

}



==> MRF/appx_special_cases.tex <==
\section{Missing Proofs about the High Temperature Regime}\label{sec:appx_special_cases}

\begin{prevproof}{Lemma}{lemma:Dobruthin properties}
$\rho_d(\vT)\leq \alpha(\vT)$ follows the elementary fact that the spectral radius is upper bounded by the infinity norm. To prove $\alpha(\vT)\leq \beta(\vT)$, we first need the following definition and lemma.
\begin{definition}\label{def:log influence}\cite{DaganDDJ19}
	Let $\bm{x}=(x_1,\ldots, x_n)$ be a random variable over $\times_{i\in[n]} \Sigma_i$, and $P_{\bm{x}}$ denote its probability distribution. Assume $P_{\bm{x}}>0$ on all $\times_{i\in[n]} \Sigma_i$. For any $i\neq j\in [n]$, define the log influence between $i$ and $j$ as $$I_{i,j}^{\log}(\bm{x})={1\over 4}\max_{\substack{x_{-i-j}\in \Sigma_{-i-j}\\ x_i, x'_i \in \Sigma_i \\ x_j,x'_j\in \Sigma_j}}\log { P_{\bm{x}}(x_i x_j x_{-i-j}) P_{\bm{x}}(x'_i x'_j x_{-i-j}) \over P_{\bm{x}}(x'_i x_j x_{-i-j}) P_{\bm{x}}(x_i x'_j x_{-i-j})}.$$
\end{definition}

\begin{lemma}[Adapted from Lemma 5.2 of~\cite{DaganDDJ19arxiv}]
	Let $\bm{x}=(x_1,\ldots, x_n)$ be a random variable , for any $i,j\in [n]$, $\alpha_{i,j}\leq I_{i,j}^{\log}(\bm{x})$. \end{lemma}

We only need to prove that $I_{i,j}^{\log}(\vT)$ is no more than $\beta_{i,j}(\vT)$. Since \argyrisnote{random variable} $\vT$ is generated by a MRF,
\begin{align*}
	I_{i,j}^{\log}(\vT)&={1\over 4}\max_{\substack{t_{-i-j}\in \Sigma_{-i-j}\\ t_i, t'_i \in \Sigma_i \\ t_j,t'_j\in \Sigma_j}}
 \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t_i,t_j,t_{-i-j}\right)_e\right) + \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t'_i,t'_j,t_{-i-j}\right)_e\right)\\
 &\qquad\qquad\qquad\qquad - \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t'_i,t_j,t_{-i-j}\right)_e\right) - \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t_i,t'_j,t_{-i-j}\right)_e\right),
\end{align*}
which is clearly no greater than $\beta_{i,j}(\vT)$.

Since for any $i,j\in[n]$ $\alpha_{i,j}\leq \beta_{i,j}(\vT)$ ,d $\alpha(\vT) \leq \beta(\vT) $.
\end{prevproof}

\input{MRF/core_trees}
\subsection{Details about the Tree Structured MRF}\label{sec:appx_tree_MRF_alg}
Assume the MRF is defined over a tree $G=(V,E)$ with only pair-wise potentials (that means that $G$ is a simple graph).
We need some additional notation.
Assume $G(V,E)$ is a tree.
For any item $u\in V$,
we denote by $C(u)$ the set of items that are children of $u$ in $G$.
Moreover when we refer to the father of item $u$,
we mean the item that is the father of item $u$ in the graph that the MRF is defined.
Similarly when we refer to the neighbors of an item $u$,
we mean its children and its parent.
In a high level idea,
the purpose of this section is to identify a metric function $d$ w.r.t. $\cup_{i\in[n]}T_i$ that minimizes the infinity norm of the $d$-Dobrushin interdependent matrix $A$ (as presented in Lemma~\ref{thm:var_d}),
so that we can effectively bound the variance of function $v(\vT,C(\vT))$.

First we need the following change in notation.
We consider the set $\E = \cup_{i \in [n]} \{(t_i,i) : t_i \in T_i\}$,
and we say that an $\vT^{\E} \in \E^n$ is valid if for each $i\in [n]$, $t_i^{\E}=(t_j,k)$ then $t_j \in T_i$ and $k=i$.
From now on,
when we refer to set $\E^n$,
we mean the subset of $\E^n$ that consists of valid elements.
We consider the following bijection mapping between $\bm{T}$ and $\E^n$: $\bm{t} \in T$ is mapped to $\bm{t}^{\E} \in \E^n$ such that $t_i^{\E} = (t_i,i)$.
We consider the MRF $D^{\E}$,
that first samples $\bm{t}\sim D$ and outputs $\bm{t}^{\E}$,
note that the structural information of the MRF $D^{\E}$ and $D$ are the same.
Similarly we define $g^{\E}(\bm{t}^{\E}):\E^n \rightarrow \mathbb{R}$ such that $g^{\E}(\bm{t}^{\E}) = v(\vT,C(\vT))$.



We need to introduce the following parameters.
Let $A^{TV}=\{\alpha^{TV}_{i,j}\}_{i,j\in[n]}$ be the $d$-Dobrushin interdependent matrix of $D$ under the trivial metric $d(t_i,t_i')=\mathds{1}_{t_i \neq t_i'}$,
that means:

\begin{align*}
    \alpha^{TV}_{i,j} =  \sup_{\substack{t_{-i},t'_{-i} \in T_{-i}, \\ t_{-i-j}, = t'_{-i-j}, t_j \neq t'_j} } d_{TV}\left(D_{i\mid t_{-i}}, D_{i\mid t_{-i}'} \right)
\end{align*}

We consider the following metric $d: \E \times \E \rightarrow \mathbb{R}$ parametrized by $v_i>0$, for $i\in[n]$:

\begin{align}
    d\left( (t_i,i), (t_i',i') \right) = 
    \begin{cases}
    v_i \mathds{1}_{t_i \neq t_i'} \quad & \text{if $i=i'$} \\
    \max_{k\in [n]}v_k \quad & \text{o.w.}
    \end{cases} \label{eq:param}
\end{align}


Note that $\alpha_{i,j}$ (as defined in Lemma~\ref{thm:var_d}) of the $d$-Dobrushin Interdependent matrix $A$ over MRF $D^{\E}$ satisfies:

\begin{align*}
    \alpha_{i,j} = & \sup_{\substack{t^{\E}_{-i},t'^{\E}_{-i} \in \E^n_{-i}, \\ t^{\E}_{-i-j}, = t'^{\E}_{-i-j}, t^{\E}_j \neq t'^{\E}_j} } \frac{W_{1,d}\left(D^{\E}_{i\mid t^{\E}_{-i}}, D^{\E}_{i\mid t'^{\E}_{-i}} \right)}{d\left((t_j,j),(t_j',j)\right)} \\
    = & \sup_{\substack{t_{-i},t'_{-i} \in T_{-i}, \\ t_{-i-j}, = t'_{-i-j}, t_j \neq t'_j} } \frac{v_i}{v_j} d_{TV}\left(D_{i\mid t_{-i}}, D_{i\mid t_{-i}'} \right) \\
    = & \frac{v_i}{v_j} \alpha^{TV}_{i,j}
\end{align*}

If $u$ is a child of $p$,
then we define $w_{(u,p)}=w_{(p,u)}= \frac{v_u}{v_p}$.
Therefore if $u$ is a child of $p$ we have that:

\begin{align*}
    \alpha_{u,p} = & w_{(u,p)} \alpha^{TV}_{u,p} \\
    \alpha_{p,u} = & \frac{1}{w_{(u,p)}} \alpha^{TV}_{p,u}
\end{align*}

%
%
%
\begin{remark}\label{remark:param}
Another way to define a metric $d$ parametrized as described in \eqref{eq:param},
is to provide a set of parameters $\{w_e\}_{e\in E}$,
where $w_{(u,p(u))}=\frac{v_u}{v_{p(u)}}$, where $p(u)$ is the parent of $u$.
Moreover the sum of the elements of the row that corresponds to item $u$ of the $d$-Dobrushin Interdependent matrix is equal to:
\begin{align*}
    w_{(u,p(u))} \alpha^{TV}_{u,p(u)} + \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}}
\end{align*}
\end{remark}
%
%
%
Now we are ready to describe how to choose the values of $w_{(u,v)}$ so that we minimize the infinity norm of the $d$-Dobrushin interdependent matrix $A$.
Assume that $k^*$ is the minimum value of the infinity norm of the $d$-Dorbushin interdependent matrix  $A$, where $d$ is parametrized as described in \eqref{eq:param}. We are going to provide a greedy algorithm,
that given a prediction $k$ about the value of $k^*$,
outputs if $k=k^*$,
if $k>k^*$ or if $k< k^*$.
The algorithm is presented in Algorithm~\ref{algo:min_norm}.


\begin{algorithm}[H] 
\caption{Given a MRF $D$ and over a tree $G(V,E)$, access to the $d$-Dobrushin interdependent matrix $A^{TV}=\{\alpha^{TV}_{i,j}\}_{i,j\in[n]}$ when $d$ is the trivial metric and a prediction $k$,
output whether $k$ is bigger, small or equal than the minimum infinity norm of the $d$-Dobrushin interdependent matrix $A$, where $d$ is parametrized as in equation~\eqref{eq:param}
}
\begin{algorithmic}\label{algo:min_norm}
 \STATE arbitrary root $G$ at item $r$
 \STATE $U\leftarrow V-\{r\}$ 
 \STATE $S\leftarrow \emptyset$ 
 \WHILE{$ U \neq \emptyset$}{
  		\STATE $u \leftarrow \text{an item in $U$ such that all of its child are in $S$}$\;
  		\IF{$k - \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} > 0$}{
   			\STATE $p \leftarrow \text{parent of $u$}$\;
   			\STATE $w_{(u,p)}\leftarrow \frac{1}{\alpha^{TV}_{u,p}} \left(k - \sum_{c \in C(u)} \frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} \right) $\;
   			\STATE $U \leftarrow U - \{u\}$\;
   			\STATE $S \leftarrow S \cup \{u\}$\;
   }
   		\ELSE {
   			\STATE Output that $k < k^*$\;
    }
    	\ENDIF
  }
  \ENDWHILE
 	\IF{$\sum_{c \in C(r)} \frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} = k $}{
 		\STATE Output that $k = k^*$\;
 	}
 	\ELSIF{$\sum_{c \in C(r)}\frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} > k $}{
 		\STATE Output that $k < k^*$\;
 	}
 	\ELSIF{$\sum_{c \in C(r)}\frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} < k $}{
 		\STATE Output that $k > k^*$\;
 	}
 	\ENDIF
 %\caption{Minimum $||A||_\infty$ value Comparator}
 \end{algorithmic}
\end{algorithm}



Intuitively,
Algorithm~\ref{algo:min_norm} use the predicted value of $k$ and tries to construct a valid metric $d$ such that the sum of elements of each row of the $d$-Dobrushin Interdependence matrix $A$ is no more than $k$.
We keep two sets of items,
one set of Explored items (the set $S$),
such that for each item $u\in S$,
we have defined the parameter $w_{(u,p)}$,
where $p$ is the parent of $u$,
and one set of Unexplored items (the set $U$) that tracks the items $u\in U$ such that we have not defined the parameter $w_{(u,p)}$,
where $p$ is the parent of $u$. The algorithm starts by exploring the items that are located at the leaves of the tree. Once we have explored all the items,
except for the root $r$,
it suffices to verify that the sum of the elements of the row of $A$ that corresponds to the root is greater, less or equal to $k$.


\begin{lemma}
\label{lem:norm_estimation}
Given a MRF $D$ over a tree $G$ and let $k^*$ be the minimum infinite norm of the $d$-Dobrushin interdependence matrix $A$ where $d$ is a metric parametrized as in \eqref{eq:param}.
Given a prediction $k$,
Algorithm~\ref{algo:min_norm} outputs whether or not $k=k^*$, $k<k^*$ or $k>k^*$ in time $O(n)$. 
\end{lemma}

\begin{proof}
First we are going to prove that the running time of the algorithm is $O(n)$.
We note that we can identify a sequence of items $u_i$,
such that for each $i$,
all the children of $u_i$ are in $\{u_j\}_{1 \leq j<i}$,
just by performing a DFS on $G$ from the root $r$,
which takes time $O(n)$.
We note that we visit the items of $G$ in the While-loop,
in a sequence like the one described above.


We also note that each item is examined at most once in the While-loop,
and each time we examine an item,
we only need to access its neighbors.
Therefore the total running time of the algorithm is $O(n)$.




Now we are going to prove the correctness of the algorithm.
Our goal is to construct a metric $d$ parametrized as in \eqref{eq:param}.
By Remark~\ref{remark:param},
it is enough to define the parameters $\{w_e\}_{e\in E}$,
where $w_{(u,p(u))}= \frac{v_u}{v_{p(u)}}$,
where $p(u)$ is the father of $u$.
First we note that each time we define a parameter $w_{(u,v)}$,
we define the entries $\alpha_{u,v}$ and $\alpha_{v,u}$ of the $d$-Dobrushin interdependent matrix $A$.
The correctness of the algorithm is based on the following observation.
Suppose we have selected item $u$ in the first step of the While-loop,
whose father is $p$.
We assign $w_{(u,p)}$,
the maximum possible value,
such that the sum of the elements of the row that corresponds to item $u$ of matrix $A$ is $k$.
Now we note that the higher the value of $w_{(u,p)}$,
the smaller the value of $\alpha_{p,u}$.
Therefore,
for each pair of items $u,v$,
where $v\in C(u)$,
the algorithm assigns the smallest value of $\alpha_{u,v}$ over any $d'$-Dobrushin matrix $A'$,
where $d'$ is another metric parametrised by \eqref{eq:param} such that the sum of the elements of the row that corresponds to $u$ is at most $k$.
Therefore when the algorithm output that $k < k^*$ in the While-loop,
it means that there is not a metric $d'$ parametrized by \eqref{eq:param} so that the $d'$-Dobrushin matrix $A$,
has infinite norm at most $k$.



After the algorithm exits the While-loop,
it means that it has defined all parameters $w_{(u,v)}$ so that for each item $u\in V-\{r\}$,
the sum of the elements of the row that corresponds to $u$ in $A$ is equal to $k$.
We also know that for any metric $d'$ as parametrised in \eqref{eq:param},
that the $d'$-Dobrushin interdependent matrix $A'$,
such that $||A'||_\infty \leq k^*$,
has for any $v \in C(r)$ $\alpha_{r,v} \leq \alpha'_{r,v}$.



Let $k_r$ be the sum of the elements of the row of $A$ that corresponds to $r$.


If $k_r > k$,
then since $\alpha_{r,u} \leq \alpha'_{r,u}$,
where $A'$ is the $d'$-Dobrushin interdependent matrix of a metric $d'$ parametrised as in \eqref{eq:param},
implies that there does not exists a metric $d'$ parametrised as in \eqref{eq:param} such that infinite norm of the $d'$-Dobrushin interdependent matrix is at most $k$.


Similarly, if $k_r = k$,
then there does not exists a metric $d'$ parametrised as in \eqref{eq:param} such that $d'$-Dobrushin interdpendent matrix $A'$ has infinity norm less than $k$.
Therefore $k^* = k$.




Finally, if $k_r < k$,
then for sufficiently small $\epsilon>0$,
if we rerun the algorithm with prediction $k-\epsilon$ (conditioning on choosing the same root in the initialization of the algorithm),
then it is going to calculate another metric $d'$ and a $d'$-Dobrushin Interdependent matrix $A'$,
such that for each item $u \in V -\{r\}$,
the sum of the elements of the row of $A'$ that corresponds to $u$ is $k-\epsilon$,
and the sum of the elements of the row of $A'$ that corresponds to $r$ is $k_r + \delta(\epsilon)$,
where $\delta(\epsilon)>0$ and $\lim_{\epsilon \rightarrow 0}\delta(\epsilon) = 0$.
Therefore $k^* \leq ||A'||_\infty < k$.


\end{proof}


\notshow{
\argyrisnote{Argyris: Should I remove them? I don't think they add anything in terms of context.}

A corollary of Lemma~\ref{lem:norm_estimation} is the following.

\begin{corollary}\label{cor:algo_output}
We can verify in time $O(n)$ using Algorithm~\ref{algo:min_norm} with prediction $k=1$ if $k^* < 1$.

If $k^* < 1$,
then using binary search with Algorithm~\ref{algo:min_norm} $\log(\epsilon)$ times,
we can approximate the value of $k^*$ within an additive $\epsilon$ term. 
The total running time of this precudure is $O(n \log(\epsilon))$
\end{corollary}


Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:var_d} and Remark~\ref{remark:sum_bound} we obtain the following Theorem:

\begin{theorem}
\label{thm:metric_var}
Given a MRF $D$ over a tree $G$ with $n$ items,
let $k^*$ be the minimum infinite norm of the $d$-Dobrushin Interdependence matrix,
where $d$ us parametrized as in \eqref{eq:param}.
For any $\epsilon>0$,
such that $k^* < 1- \epsilon$,
we can identify a metric $d$ such that the $d$-Dobrushin interdpendent matrix $A$ satisfies $||A||_\infty \leq k^* + \epsilon$ in time $O(n \log(\epsilon))$.
If we can identify such a metric $d$,
then we also have:

\begin{align*}
    Var[v(\vT,C(\vT)] \leq \frac{2(\srev)(\core)}{1-k^*-\epsilon} 
\end{align*}
\end{theorem}


}



%\subsection{Buyers valuation is a MRF over a General Class of Trees}\label{subsec:core_d_trees}
\subsection{Proof of Lemma~\ref{lemma:tree_sufficient_condition}}\label{subsec:core_d_trees}
\begin{prevproof}{Lemma}{lemma:tree_sufficient_condition}
The proof of the lemma is directly inspired by Algorithm~\ref{algo:min_norm}.
Let $d$ be a metric parametrized as described in \eqref{eq:param},
then according to Remark~\ref{remark:param} it is enough to define parameters $\{w^*_e\}_{e\in E}$.
Let $A$ be the $d$-Dobrushin interdependent matrix of $\vT$,
under the metric $d$ we just described, where for each $e\in E$ we set $w^*_e = w_e$.
Let $A^{TV}=\{a^{TV}_{u,v}\}_{u,v\in V}$ be the $d$-Dobrushin interdependent matrix of $\vT$ under the trivial metric.
By Lemma~\ref{lemma:Dobruthin properties} we have that $\alpha^{TV}_{u,v} \leq \beta_{u,v}$.
Therefore the sum of elements of the row that corresponds to item $u$ of $A$ can be bounded by:
\begin{align*}
w_{(p(u),u)} \alpha^{TV}_{p(u),u} + \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} \leq w_{(p(u),u)} \beta_{p(u),u} + \sum_{c \in C(u)}\frac{\beta_{u,c}}{w_{(u,c)}} \leq k(\vT)    
\end{align*}

The inequality above implies that the infinity norm of $A$ is upper bounded by $k(\vT)$.
Since the spectral radius of $A$ is upper bounded by the infinity norm of $A$,
we conclude that $\rho_d(\vT) \leq k(\vT)$.
\end{prevproof}

\notshow{
\argyrisnote{Argyris: I believe we should erase the rest of this section.}


In this section we are going to demonstrate how we can use Lemma~\ref{lem:norm_estimation} in order to provide a condition such that we can efficiently bound the covariance of $v(\vT,C(\vT))$,
when the buyers valuation is a MRF but does not satisfies the Dobrushin Uniqueness Condition.
We assume that the MRF $D$ is over a Tree and there exists a parameter $w\in \mathbb{R}_+$,
such that $k=\max_{\substack{u \in V,\\ \text{$p$ father of $u$}}}w \beta_{u,p} + \frac{1}{w}\sum_{c \in C(u)}\beta_{u,c} < 1$.
We are going to show that are instances of trees in this category where the inverse temperature of the MRF could be arbitrary large,
and violate the Dobrushin Uniqueness Condition.



We are going to prove that there exists a metric $d$, parametrized as in \eqref{eq:param} such that infinity norm of the $d$-Dobrushin Interdependent matrix is bounded by $k$ (This prediction is a generalization of \cite{levin2017markov}, Section~15.4, Theorem~15.6).




\begin{lemma} \label{lem:tree_metric}
Given a MRF $D$ over a tree $G(V,E)$ and a parameter $w\in \mathbb{R}_+$,
let $k=\max_{\substack{u \in V,\\ \text{$p$ father of $u$}}}w \beta_{u,p} + \frac{1}{w}\sum_{c \in C(u)}\beta_{u,c} < 1$,
then running Algorithm~\ref{algo:min_norm} with prediction $k$,
outputs that there exists a metric $d$ such that the infinite norm of the $d$-Dobrushin Interdependent matrix is bounded by $k$.
\end{lemma}
\yangnote{Why do we need to set $w$ to be the same for each edge? Why do we need the algorithm to prove this claim? It follows from the definition, no?}
\begin{proof}
First we assume that root of $G$ is the same as the root selected in Algorithm~\ref{algo:min_norm}.
We are going to prove by induction that between any pair of items $u,p$, where $p$ is the parent of $u$,
$w_{(u,p)}\geq w$ (this statement does not cover the case where $u$ is the root of the tree).


In order to prove the base case,
it is enough to prove that the induction hypothesis holds for the leafs of $G$.
Let $u$ be a leaf and $p$ its parent,
noting that $w \beta_{u,p} \leq k$,
the algorithm makes the following assignment:

\begin{align*}
    w_{(u,p)} \leftarrow \frac{k}{\beta_{u,p}} \geq w
\end{align*}

Therefore the base case is now settled.

For the induction step,
we assume that we visit an item $u$ such that for each $c \in C(u)$,
it holds that $w_{(u,c)} \geq  w$.
Let $p$ be the parent of $u$,
Algorithm~\ref{algo:min_norm} makes the following assignment:
\begin{align*}
    w_{(u,p)} \leftarrow & \frac{1} {\beta_{u,p}} \left( k - \sum_{c\in C(u)}\frac{\beta_{c,u}}{w_{c,u}} \right) \\
    \geq & \frac{1} {\beta_{u,p}} \left( k - \frac{1}{w}\sum_{c\in C(u)}\beta_{c,u} \right) \\
    \geq & \frac{1} {\beta_{u,p}}  w \beta_{u,p}  \\
    = & w
\end{align*}

The last inequality holds by the definition of $k$.
Therefore for any edge $(u,v)\in E$,
Algorithm~\ref{algo:min_norm} assignes $w_{(u,v)} \geq w$.
This fact implies that the Algorithm~\ref{algo:min_norm} does not output $k<k^*$ on the While-Loop.


Now we turn our attention to the root $r$.
It is enough now to verify that $\sum_{c \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} < k $,
which would imply that $k > k^*$ and we can conclude the proof.
Noting that $w_{(u,v)} \geq w$ for each $(u,v)\in E$:
\begin{align*}
    \sum_{c  \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} \leq \frac{1}{w}\sum_{c \in C(r)}\beta_{r,c}  \leq k
\end{align*}


\end{proof}


We make the following observation.

\begin{observation}\label{obs:specific_metrics}
If we apply Lemma~\ref{lem:tree_metric} with $w=1$,
then the value of $k$ is equal to the inverse temperature of $D$.


If we consider the case where $G(V,E)$ is the complete $d$-ary tree,
such that for each $(u,v)\in E$, $\beta_{u,v} \leq \beta < \frac{1}{2\sqrt{d}}$,
then for each node $u\in V$ it holds that:
\begin{align*}
    \sqrt{d}\beta_{u,p} + \frac{1}{\sqrt{d}} \sum_{c \in C(u)}\beta_{u,c} < 1
\end{align*}

Therefore we can apply Lemma~\ref{lem:tree_metric} on $D$ with parameter $w=\sqrt{d}$ and prediction $k=2\sqrt{d} \beta$.

We note that the inverse temperature in this case could be as high as $\frac{\sqrt{d}}{2}$ which would violate the Dobrushin condition.
\end{observation}


%Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:metric_var} and Observation~\ref{obs:specific_metrics} we obtain the following result.

}




\notshow{

In this section we are going to demonstrate how we can use Lemma~\ref{lem:norm_estimation} in order to provide a condition such that we can efficiently bound the covariance of $v(\vT,C(\vT))$,
when the buyers valuation is a MRF but does not satisfies the Dobrushin Uniqueness Condition.
We assume that the MRF $D$ is over a $d$-ary Tree where each pairwise-potential is bounded by $\beta\leq \frac{1}{2\sqrt{d}}$.
Note the inverse temperature of this MRF could be as high as $\frac{\sqrt{d}}{2}$,
which would violate the Dobrushin Uniqueness Condition.



We are going to prove that there exists a metric $d$, parametrized as in \eqref{eq:param} such that infinity norm of the $d$-Dobrushin Interdependent matrix is bounded by $2 \beta \sqrt{d}$ (This prediction is based on \cite{levin2017markov}, Section~15.4, Theorem~15.6).



\begin{lemma} \label{lem:tree_metric}
Given a MRF $D$ over a $d$-ary tree $G(V,E)$ such that the Markov influence between any pair of items is bounded by $\beta$,
then running Algorithm~\ref{algo:min_norm} with prediction $k=2\beta \sqrt{d}$,
conditioned on the fact that the root of $G$ is the same as the root selected in Algorithm~\ref{algo:min_norm},
outputs that there exists a metric $d$ such that the infinite norm of the $d$-Dobrushin Interdependent matrix is bounded by $2\beta \sqrt{d}$.
\end{lemma}

\begin{proof}
First we are going to prove by induction that between any pair of items $u,p$, where $p$ is the parent of $u$,
$w_{(u,p)}\geq \sqrt{d}$ (this statement does not cover the case where $u$ is the root the $d$-ary tree).


In order to prove the base case,
it is enough to prove that the induction hypothesis holds for the leafs of $G$
Let $u$ be a leaf and $p$ its parent,
the algorithm makes the following assignment:

\begin{align*}
    w_{(u,p)} \leftarrow \frac{2 \sqrt{d} \beta}{\beta_{u,v}} \geq 2 \sqrt{d}
\end{align*}

Therefore the base case is now settled.

For the induction step,
we assume that we visit an item $u$ such that for each $c \in C(u)$,
it holds that $w_{(u,c)} \geq  \sqrt{d}$.
Let $p$ be the parent of $u$,
Algorithm~\ref{algo:min_norm} makes the following assignment:
\begin{align*}
    w_{(u,p)} \leftarrow & \frac{1} {\beta_{u,p}} \left( 2 \beta \sqrt{d} - \sum_{c\in C(u)}\frac{\beta_{c,u}}{w_{c,u}} \right) \\
    \geq & \frac{1} {\beta} \left( 2 \beta \sqrt{d} - \sum_{c\in C(u)}\frac{\beta}{w_{c,u}} \right) \\
    \geq &  \left( 2 \sqrt{d} - \sum_{c\in C(u)}\frac{1}{\sqrt{d}} \right) \\
    = & \left( 2 \sqrt{d} - \frac{d}{\sqrt{d}} \right) = \sqrt{d}\\
\end{align*}

Therefore for any edge $(u,v)\in E$,
Algorithm~\ref{algo:min_norm} assignes $w_{(u,v)} \geq \sqrt{d}$.
This fact implies that the Algorithm~\ref{algo:min_norm} does not output $k<k^*$ on the While-Loop.


Now we turn our attention to the root $r$.
It is enough now to verify that $\sum_{c \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} < 2\beta \sqrt{d} $,
which would imply that $k > k^*$ and we can conclude the proof.
We note that according to the fact that $w_{(u,v)} \geq \sqrt{d}$ for each $(u,v)\in E$:
\begin{align*}
    \sum_{c  \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} \leq \sum_{c \in C(r)}\frac{\beta}{\sqrt{d}}  = \sqrt{d} \beta < 2\sqrt{d}\beta
\end{align*}


\end{proof}



Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:metric_var} and Lemma~\ref{lem:tree_metric} we obtain the following result.




\begin{lemma}

Let the type distribution $D$ be a MRF such that the corresponding graph is a complete $d$-ary tree and the value of the Markov influence between any pair of items is bounded by $\beta < \frac{1}{2\sqrt{d}}$.
Then:

\begin{align*}
    Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1- 2\sqrt{d}\beta} 
\end{align*}
\end{lemma}

}

==> MRF/appx_special_cases_ec.tex <==
\section{Missing Details from Section~\ref{sec:Dobrushin}}\label{sec:appx_special_cases}
\argyrisnote{I moved the proofs from this section to the main body}


\begin{prevproof}{Lemma}{lem:Dobrushin implies large spectral gap}
By Lemma~\ref{lem:Poincare on MRF},
there exists a function $g^*:\Omega\rightarrow \mathbb{R}$, such that
$$   \frac{\sum_{i \in [n]}  \E_{\vT \sim D} \left[ \left( g^*(t_i,\vT_{-i}) - \E_{t'_i \sim D_{i \mid \vT_{-i}}}[g^*(t'_i,\vT_{-i})] \right)^2 \right]}{\Var_{\vT\sim D}[g^*(\vT)]} = n\gamma.$$

The following result by Wu~\cite{wu2006} provides a generalization of the Efron-Stein inequality for \emph{weakly dependent random variables}.

\begin{lemma}[Poincar\'{e} Inequality for Weakly Dependent Random Variables - Theorem~2.1 in \cite{wu2006}]
\label{thm:var_d}
Let $\vT=(t_1,\ldots,t_n)$ be an $n$-dimensional random vector drawn from distribution $D$ that is supported on $\E^n$. For any metric $d(\cdot,\cdot)$ on $\E$, let $A$ be the $d$-Dobrushin interdependence matrix for $\vT$. Let $\rho_d(\vT)$ be the spectral radius of $A$. If $\E_{\vT \sim D}\left[ \sum_{i\in[n]} d(t_i,y_i)^2 \right] < + \infty$ for some fixed $y \in \E^n$ and  $\rho_d(\vT) < 1$, then for any square integrable function $g(\cdot)$ w.r.t. distribution $D$, the following holds:
$$    (1-\rho_d(\vT))\Var_{\vT\sim D}[g(\vT)] \leq \sum_{i \in [n]} \E_{\vT \sim D} \left[  \left( g(t_i,\vT_{-i}) - \E_{t_i' \sim D_{i \mid \vT_{-i}}}[g(t_i,\vT_{-i})] \right)^2 \right] .$$
\end{lemma}

If we choose $g(\cdot)$ to be $g^*(\cdot)$ in Lemma~\ref{thm:var_d},
we have that :
$$    1-\rho_d(\vT)\leq \frac{\sum_{i \in [n]} \E_{\vT \sim D} \left[  \left( g^*(t_i,\vT_{-i}) - \E_{t_i' \sim D_{i \mid \vT_{-i}}}[g^*(t_i,\vT_{-i})] \right)^2 \right]}{\Var_{\vT\sim D}[g^*(\vT)] }$$

Combining the two inequalities conclude the proof
\end{prevproof}


\begin{prevproof}{Lemma}{lemma:Dobruthin properties}
$\rho_d(\vT)\leq \alpha(\vT)$ follows the elementary fact that the spectral radius is upper bounded by the infinity norm. To prove $\alpha(\vT)\leq \beta(\vT)$, we first need the following definition and lemma.
\begin{definition}\label{def:log influence}\cite{DaganDDJ19}
	Let $\bm{x}=(x_1,\ldots, x_n)$ be a random variable over $\times_{i\in[n]} \Sigma_i$, and $P_{\bm{x}}$ denote its probability distribution. Assume $P_{\bm{x}}>0$ on all $\times_{i\in[n]} \Sigma_i$. For any $i\neq j\in [n]$, define the log influence between $i$ and $j$ as $$I_{i,j}^{\log}(\bm{x})={1\over 4}\max_{\substack{x_{-i-j}\in \Sigma_{-i-j}\\ x_i, x'_i \in \Sigma_i \\ x_j,x'_j\in \Sigma_j}}\log { P_{\bm{x}}(x_i x_j x_{-i-j}) P_{\bm{x}}(x'_i x'_j x_{-i-j}) \over P_{\bm{x}}(x'_i x_j x_{-i-j}) P_{\bm{x}}(x_i x'_j x_{-i-j})}.$$
\end{definition}

\begin{lemma}[Adapted from Lemma 5.2 of~\cite{DaganDDJ19arxiv}]
	Let $\bm{x}=(x_1,\ldots, x_n)$ be a random variable , for any $i,j\in [n]$, $\alpha_{i,j}\leq I_{i,j}^{\log}(\bm{x})$. \end{lemma}

We only need to prove that $I_{i,j}^{\log}(\vT)$ is no more than $\beta_{i,j}(\vT)$. Since {random variable} $\vT$ is generated by a MRF,
\begin{align*}
	I_{i,j}^{\log}(\vT)&={1\over 4}\max_{\substack{t_{-i-j}\in \Sigma_{-i-j}\\ t_i, t'_i \in \Sigma_i \\ t_j,t'_j\in \Sigma_j}}
 \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t_i,t_j,t_{-i-j}\right)_e\right) + \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t'_i,t'_j,t_{-i-j}\right)_e\right)\\
 &\qquad\qquad\qquad\qquad - \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t'_i,t_j,t_{-i-j}\right)_e\right) - \sum_{\substack{e \in E :\\ i,j \in e}} \psi_e\left(\left(t_i,t'_j,t_{-i-j}\right)_e\right),
\end{align*}
which is clearly no greater than $\beta_{i,j}(\vT)$.

Since for any $i,j\in[n]$ $\alpha_{i,j}\leq \beta_{i,j}(\vT)$, we have $\alpha(\vT) \leq \beta(\vT) $.
\end{prevproof}



==> MRF/core.tex <==
\subsubsection{Bounding the \core~using the Poincar\'{e} Inequality}\label{sec:XOS_core}

In this section, we show how to bound the \core~for an XOS buyer. The $\core$ is the expectation of the random variable $v(\vT,C(\vT))$. To show that bundling can achieve a good approximation of the \core, we need to upper bound the variance of $v(\vT,C(\vT))$. This is the main technical task for this section. As $v(\vT,\cdot)$ is not additive across the items, our method for the additive valuation (see Lemma~\ref{lemma:cov}) no longer applies. We provide a new approach that is based on the \emph{Poincar\'{e} Inequality}~\cite{wu2006} and the \emph{self-boundingness of XOS functions}. We first provide the necessary notation and techniques.


\begin{definition}[Self-Bounding Functions~\cite{BoucheronLM00}]\label{def:self-bounding}
We say that a function $g(\vT): \mathbb{E}^n \rightarrow \mathbb{R}$,
where $\E$ can be any set,
is \emph{$C$-self-bounding} with some constant $C\in \mathbb{R}_+$ if there exists functions $g_i:\E^{n-1}\rightarrow \mathbb{R}$ for all $i\in[n]$ such that for each $\vT \in \E^n$ the followings hold:
\begin{itemize}
    \item $0 \leq g(\vT)-g_i(\vT_{-i}) \leq C$ for all $i\in[n]$.
    \item $\sum_{i\in[n]} \left(g(\vT)-g_i(\vT_{-i})\right)\leq g(\vT)$. 
\end{itemize}


\end{definition}



Next, we prove that $g(\vT)=v(\vT,C(\vT))$ is $2\srev$-self-bounding. Recall that $C(\bm{t}) = \{ j : V_j(\bm{t}) < 2 \srev\}$.

\begin{lemma}
\label{lemma:self_bounding_MRF}
The function $g(\vT)=v(\vT,C(\vT))$ is $2\srev$-self-bounding.
\end{lemma}

\begin{proof}
Define $g_i(\vT_{-i}) = v(\vT_{-i},C(\vT_{-i}))$, where $C(\vT_{-i})=\{ j : V_j(\bm{t_{-i}}) < 2 \srev\}$. When $i\notin C(\vT)$, $g(\vT)-g_i(\vT_{-i})= 0$. When $i\in C(\vT)$, $C(\vT)=C(\vT_{-i})\cup \{i\}$. Additionally, $g(\vT)-g_i(\vT_{-i})\geq 0$ and $g(\vT)-g_i(\vT_{-i})\leq V_i(\vT)\leq 2\srev$.  Since $v(\cdot,\cdot)$ is an XOS function, there exists non-negative numbers $\{x_\ell\}_{\ell \in C(\vT)}$ such that $g(\vT) = \sum_{\ell\in C(\vT)} x_\ell$ and $g_i(\vT_{-i}) \geq \sum_{\ell\in C(\vT_{-i})} x_\ell$. Therefore, $\sum_{i\in[n]} \left(g(\vT)-g_i(\vT_{-i})\right)\leq \{x_\ell\}_{\ell \in C(\vT)}= g(\vT)$.
%Let $\bm{t}\in \bm{T}$. Let $j^*= arg\max_{j \in [k]} \sum_{i \in C(\bm{t})} t^{(j)}_i$. This implies that $v(\vT,C(\vT))=\sum_{i \in C(\bm{t})} t^{(j^*)}_i$. We consider the functions $b_i(\bm{t})=t^{(j^*)}_i  \mathds{1}[0 \leq V_i(\vT) \leq 2\bm{SRev}]$. We note that $t^{(j^*)}_i \leq V_i(t_i)$. Therefore we have that:

%\begin{align*}
 %   0 \leq b_i(\bm{t}) \leq 2 (\srev) \\
  %  \sum_{i \in [n]} b_i(\bm{t}) = v(\vT,C(\vT))
%\end{align*}



%We now consider $\bm{t},\bm{t'} \in \bm{T}$.
%then their difference is at most when %t_{i_1}'=t_{i_2}'=\ldots=t_{i_k}'=0$.
%We note that $v(\bm{t'},C(\bm{t'}))\geq \sum_{i \in C(\bm{t}')} t'^{(j^*)}_i \geq \sum_{i \in C(\bm{t}') :t_i'=t_i} t'^{(j^*)}_i$.
%Therefore we have that:

%\begin{align*}
%v(\bm{t},C(\bm{t}))-v(\bm{t'},C(\bm{t}')) \leq &\sum_{i: t_i \neq t_i'} t^{(j^*)}_i \mathds{1}[0 \leq V_i(t_i) \leq 2\bm{SRev}] = \sum_{i: t_i \neq t_i'} b_i(\bm{t})
%\end{align*}

%We proved that all three properties of the self-bounding function are satisfied.
%This concludes the proof.
\end{proof}


%Now we are going to provide a Theorem from \cite{wu2006} that helps us bound the $(\core)$.
To state the Poincar\'{e} Inequality, we first introduce the notion of \emph{Dobrushin's Interdependence Matrix}.

\begin{definition}[$d$-Dobrushin Interdependence Matrix~\cite{wu2006}]\label{def:Dobrushin's interdependence matrix}
Let $(\E,d)$ be a metrical, complete and separable space.
For two distributions $\mu$ and $\nu$ supported on $\E$,
their $L^1$-Wasserstein distance is defined as:    $$W_{1,d}(\mu,\nu) = \inf_{\pi \in \Pi} \int\int_{\E \times \E} d(x,y) \pi(dx,dy),$$ where $\Pi$ is the set of valid coupling such that its marginal distributions are $\mu$ and $\nu$. If we choose $d(x,y)$ to be the trivial metric $\ind_{x\neq y}$, then $W_{1,d}(\cdot,\cdot)$ is exactly the total variation distance.
Let $X=(x_1,\ldots, x_n)$ be a $n$-dimensional random vector supported on $\E^n$ and $\mu_i(\cdot \mid x_{-i})$ be the conditional distribution of $x_i$ knowing $x_{-i}$. Define the \textbf{$d$-Dobrushin Interdependence Matrix} $A=(\alpha_{i,j})_{i,j\in[n]}$ by
$$\alpha_{i,j}:= \sup_{\substack{x_{-i-j}=y_{-i-j}\\ x_j\neq y_j}}\frac{W_{1,d}(\mu_i(\cdot\mid x_{-i}),\mu_i(\cdot\mid y_{-i}))}{d(x_j,y_j)}.$$
\end{definition}
\begin{remark}
$\alpha_{i,j}$ captures how strong the value of $x_j$ affects the conditional distribution of
$x_i$ when all other coordinates are fixed. Higher $\alpha_{i,j}$ value implies stronger dependence between $x_i$ and $x_j$. When all the coordinates of $X$ are independent, $A$ is the all zero matrix. 
\end{remark}
Now we are ready to present the Poincar\'e inequality. Very high-levelly speaking, Poincar\'{e} inequalities connect the variance of a function $g(\cdot)$ with the $\ell_2$-norm of the gradient of $g(\cdot)$, and usually take the form of $\Var_{X\sim D}[g(X)]\lesssim\E_{X\sim D}[||\text{gradient}(g(X))||^2]$. These inequalities are called \emph{Poincar\'e inequalities} because Poincar\'{e} first published an inequality of this type for the uniform distribution on a bounded domain in $\mathbb{R}^n$, ca. 1890. Many similar inequalities have since been discovered. One notable example is the Efron-Stein inequality~\cite{efron1981jackknife}, which has numerous applications in combinatorics, statistics, and statistical learning~\cite{massart2007concentration,boucheron2013concentration}. The Efron-Stein inequality only applies to \emph{independent random variables}. The following lemma by Wu~\cite{wu2006} provides a generalization of the Efron-Stein inequality for \emph{weakly dependent random variables}.

\begin{lemma}[Poincar\'{e} Inequality for Weakly Dependent Random Variables \cite{wu2006}]
\label{thm:var_d}
Let $\vT=(t_1,\ldots,t_n)$ be an $n$-dimensional random vector drawn from distribution $D$ that is supported on $\E^n$. For any metric $d(\cdot,\cdot)$ on $\E$, let $A$ be the $d$-Dobrushin interdependence matrix for $\vT$. Let $\rho_d(\vT)$ be the spectral radius of $A$ (which is the dominant eigenvalue of $A$ by the Perron-Frobenius Theorem).
If $\E_{\vT \sim D}\left[ \sum_{i\in[n]} d(t_i,y_i)^2 \right] < + \infty$ for some fixed $y \in \E^n$ and  $\rho_d(\vT) < 1$, then for any square integrable function $g(\cdot)$ w.r.t. distribution $D$, the following holds:
$$    (1-\rho_d(\vT))\Var_{\vT\sim D}[g(\vT)] \leq \sum_{i \in [n]} \E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( f(t_i,\vT_{-i}) - \E_{t_i \sim D_{i \mid \vT_{-i}}}[f(t_i,\vT_{-i})] \right)^2 \right] \right].$$
\end{lemma}

\begin{remark}
In the independent case, $\rho_d(\vT)=0$, which recovers the Efron-Stein inequality. The condition that $\rho_d(\vT)<1$ is a natural condition. Firstly, it is implied by a well-known concept known as the \textbf{Dobrushin uniqueness condition} (see Section~\ref{subsec:core_dob} for more discussion) that can has been used to model weakly dependent random variables~\cite{DaganDDJ19}. Secondly, the condition implies rapid mixing of the Glauber dynamics (see Lemma~\ref{lemma:rapid mixing}). Note that a special case of Lemma~\ref{lemma:rapid mixing}, where $d(x,y)=\ind_{x\neq y}$, was shown by Hayes~\cite{Hayes06}. %We provide the general case here for completeness. %related to the $d$-Dobrushin interdependence matrix is the \textbf{Dobrushin uniqueness condition}, which was originally introduced by Dobrushin~\cite{Dobruschin68} in the study of Gibbs measures, in the context of identifying conditions under which the Gibbs distribution has a unique equilibrium. Since then, the model has been extensively studied in statistical physics and probability literature (see e.g.~\cite{DobrushinS87,StroockZ92}). The Dobrushin uniqueness condition can also be %implies a number of desirable properties, such as fast mixing of Glauber dynamics~\cite{Kulske03}, concentration of measure~\cite{Chatterjee05, Daskalakis18,Gheissari18,Kulske03,Marton96}, and correlation decay~\cite{Kunsch82}, and has been used as . For a survey of properties resulting from Dobrushin's condition see~\cite{Weitz05}. We plan to investigate the following question.

\end{remark} 


Although the RHS of the Poincar\'{e} inequality may seem complicated, we show that it can be  upper bounded by $O(\E[g(\vT)])$ when $g(\cdot)$ is a self-bounding function.
\begin{lemma} \label{lemma:sum_bound}
Let $g$ be a $C$-self-bounding function.
Then:
\begin{align*}
    \sum_{i \in [n]} \E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - \E_{t'_i \sim D_{i \mid \vT_{-i}}}[g(t'_i,\vT_{-i})] \right)^2 \right] \right] \leq C \E_{\vT \sim D} \left[ g(\vT) \right]
\end{align*}
\end{lemma}

\begin{proof}
 Recall the following property of the variance: for any real-value random variable $X$, $\Var[X]=\min_{a\in R} \E[(X-a)^2]$. In other words, $\Var[X]\leq \E[(X-a)^2]$ for any $a$. Therefore, for any $\vT_{-i}$, $$\E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - \E_{t'_i \sim D_{i \mid \vT_{-i}}}[g(t'_i,\vT_{-i})] \right)^2\right] = \Var[g(\vT)\mid \vT_{-i}]\leq \E_{t_i \sim D_{i \mid \vT_{-i}}} \left[ \left( g(\vT) - g_i(\vT_{-i}) \right)^2\right].$$ 
 
Using this relaxation, we proceed to prove the claim.
\begin{align*}
    & \sum_{i \in [n]}\E_{\vT_{-i} \sim D_{-i}} \left[ \E_{t_i \sim D_{i \mid t_{-i}}} \left[ \left( f(t_i,t_{-i}) - \E_{t_i \sim D_{i \mid t_{-i}}}[f(t_i,t_{-i})] \right)^2 \right] \right] \\
    \leq & \sum_{i \in [n]}\E_{\vT \sim D} \left[ \left( g(\vT) - g_i(\vT_{-i}) \right)^2 \right] \\
    \leq & C \sum_{i \in [n]}\E_{\vT \sim D} \left[ \left(g(\vT) - g_i(\vT_{-i})\right) \right] \\
    \leq & C \E_{\vT \sim D} \left[ g(\vT) \right]
\end{align*}

\end{proof}
\notshow{
Therefore,
if we want to bound the variance of  $v(\vT,C(\vT))$,
when its input is sampled from a MRF $D$,
it is enough to define a metric $d$,
such that the infinite norm of the $d$-Dobrushin interdependence matrix of $D$ (as defined in Theorem~\ref{thm:var_d}) is less than $1$.


The goal of the following subsections is to use the flexibility that Theorem~\ref{thm:var_d} provides us to define a metric $d$  so that we can derive meaningful bounds for the variance of $v(\vT,C(\vT))$.

\subsubsection{Putting Everything Together}


We can unify the bounds derived in Subsection~\ref{subsec:core_dob}, Subsection~\ref{subsec:core_trees} and Subsection~\ref{subsec:core_d_trees} for the variance of $v(\vT, C(\vT))$ by considering a variable $c\in [0,1\}$ (that depends on the MRF $D$ that we consider) such that $Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1 - c}$.

}

Now, we show how to approximate $\core$ using $\srev$ and $\brev$.

\begin{lemma}\label{lemma:XOS_core}
%Let $D$ be a MRF such that $Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1- c}$,
Let $d(\cdot,\cdot)$ be a metric and $\rho_d(\vT)$ be  the spectral radius of the $d$-Dobrushin interdependence matrix of $\vT$. If $\rho_d(\vT)\in[0,1)$, then $\Var[v(\vT,C(\vT))] \leq \frac{2\srev\cdot \core}{1 - \rho_d(\vT)}$. Moreover,
$$\core \leq \max\left( \frac{4\srev}{\sqrt{1-\rho_d(\vT)}} ,\left(7 + \frac{4}{\sqrt{1-\rho_d(\vT)}} \right)\brev \right).$$
\end{lemma}
\begin{proof}
According to Lemma~\ref{lemma:self_bounding_MRF}, $v(\vT,C(\vT))$ is a $2\srev$-self-bounding function. Combining Lemma~\ref{thm:var_d} and Lemma~\ref{lemma:sum_bound}, we can further show that $\Var[v(\vT,C(\vT)]\leq \frac{2\srev\cdot \E_{\vT\sim D}[v(\vT,C(\vT)]}{1-\rho_d(\vT)}=\frac{2\srev\cdot \core}{1-\rho_d(\vT)}$.

If $\core \leq \frac{4\srev}{\sqrt{1-\rho_d(\vT)}}$,
then the statement holds. If $\core > \frac{4\srev}{\sqrt{1-\rho_d(\vT)}}$,
then $\Var[v(\vT,C(\vT))] \leq \frac{2\core\cdot \srev}{1-\rho_d(\vT)} <  \frac{(\core)^2}{2\sqrt{1-\rho_d(\vT)}} = \frac{ \E[v(\vT,C(\vT))]^2}{2\sqrt{1-\rho_d(\vT)}}$.
By Paley-Zygmund inequality we have that:
    $$ \Pr\left[ v(\bm{t},C(\bm{t})) \geq \frac{\core}{3}  \right] 
    \geq \frac{4}{9} \frac{1}{1 + \frac{Var[v(\vT,C(\vT))]}{\E[v(\vT,C(\vT))]^2}} 
    \geq  \frac{4}{9} \frac{1}{1 + \frac{1}{2\sqrt{1-\rho_d(\vT)}}} .$$
Therefore we have that: $\Pr\left[ v(\bm{t},C(\bm{t})) \geq \frac{\core}{3}  \right]\cdot \frac{\core}{3} \leq \brev$, which implies that $$ \core \leq \frac{27}{4}\left(1 + \frac{1}{2\sqrt{1-\rho_d(\vT)}}\right)\brev \leq \left(7 + \frac{4}{\sqrt{1-\rho_d(\vT)}}\right) \brev.$$

\end{proof}

Finally, we combine our analysis of \single, \tail, and \core~to obtain the approximation guarantee for an XOS buyer.
\begin{theorem}\label{thm:XOS}
 Let the buyer's type $\vT$ be generated by a MRF $D$. If there exists metric $d(\cdot,\cdot)$ such that $\rho_d(\vT)\in[0,1)$, then for any XOS valuation $v$, the revenue obtained by any IC mechanism $M$ is bounded by: 
    $$\rev(M,v, D)\leq  12\exp(12\Delta(\vT)) \cdot \srev + \left(28 + \frac{16}{\sqrt{1-\rho_d(\vT)}}\right)\max\{\srev,\brev\}.$$ 
\end{theorem}
\begin{prevproof}{Theorem}{thm:XOS}
The statement follows from the combination of Lemma~\ref{lemma:XOS_single_tail} and Lemma~\ref{lemma:XOS_core}.
\end{prevproof}


%where $c = \alpha^M$ if the MRF $D$ satisfies the Dobrushin Uniqueness Condition, or $c = 2\beta \sqrt{d}$ if the MRF $D$ is over a $d$-ary tree such that the highest value of the Markov Correlation for any pair of items is bounded by $\beta < \frac{1}{2\sqrt{d}}$.







==> MRF/special_cases.tex <==
%\section{Application to Special MRFs}\label{sec:special MRF}
%We apply our general approximation results to special MRFs.

\notshow{This condition is the well-known Dobrushin Uniqness condition.
We make the following remark:

\begin{remark} \label{remark:reverse_temperature}
Let $E= \cup_{i \in [n]} T_i $.
If we define the metric $d:E\times E \rightarrow \mathbb{R}$ such that $d(x,y)=\mathds{1}[x,y]$,
then we note that the $d$-Dobrushin interdependence matrix $A$ of type distribution $D$ has the following property:

\begin{align*}
    \alpha_{i,j} = \beta_{i,j}
\end{align*}

where $\beta_{i,j}$ is the Markov influence from item $i$ to item $j$.

Let $\rho_d(\vT)$ be the spectral radius of $A$.
Then $\rho_d(\vT) \leq ||A||_\infty = \beta$.
\end{remark}


By combining Theorem~\ref{thm:var_d}, Remark~\ref{remark:sum_bound} and Remark~\ref{remark:reverse_temperature} we have the following lemma.}


\notshow{\subsection{Dobrushin's Condition~\cite{dobruschin1968}}\label{sec:Dobrushin}
\begin{definition}[Influence and the Dobrushin's Coefficient]\label{def:influence and dobrushin}
Let $\bm{x}= \left(x_1, \ldots,  x_n \right)$ be a random variable,
where each $x_i$ is supported on an alphabet $\Sigma_i$.
We define the \textbf{influence} of random variable $x_j$ over random variable $x_i$ as:
\begin{align*}
	I_{j \rightarrow i}(\bm{x}) = \max_{  \substack{ z_{-i-j} \in \Sigma_{-i-j} \\ z_j,z'_j \in \Sigma_j } } 
	%
	d_{TV} \left( P_{x_i\mid x_{-i}}\left( \cdot \mid z_{-i-j},~ z_j \right) , P_{x_i\mid x_{-i}}\left( \cdot \mid z_{-i-j},~z'_j \right)   \right)
\end{align*}

where $P_{x_i\mid x_{-i}}(\cdot\mid z_{-i})$ denotes the distribution of the random variable $x_i$ conditioned on $x_{-i} = z_{-i}$.
Moreover, we define the \textbf{Dobrushin's coefficient} of $\bm{x}$ as:
\begin{align*}
	\alpha(\bm{x}) = \max_{i\in[n]} \sum_{j \neq i} I_{j \rightarrow i}(\bm{x}).
\end{align*}
\end{definition}

\yangnote{Redefine the Dobrushin's coefficient as Wasserstein distance under any general metric. Say the current version is using the Hamming metric.}
 
The next lemma shows the relation between the Markov influence and influence, which implies the relation between the temperature of a MRF and its corresponding Dobrushin's coefficient.








In this subsection,
we consider that the type distribution $D$ of the buyer is a MRF with inverse temperature $\beta < 1$.
This condition is the well-known Dobrushin Uniqness condition.
We make the following remark:

\begin{remark} \label{remark:reverse_temperature}
Let $E= \cup_{i \in [n]} T_i $.
If we define the metric $d:E\times E \rightarrow \mathbb{R}$ such that $d(x,y)=\mathds{1}[x,y]$,
then we note that the $d$-Dobrushin interdependence matrix $A$ of type distribution $D$ has the following property:

\begin{align*}
    \alpha_{i,j} = \beta_{i,j}
\end{align*}

where $\beta_{i,j}$ is the Markov influence from item $i$ to item $j$.

Let $\rho$ be the spectral radius of $A$.
Then $\rho \leq ||A||_\infty = \beta$.
\end{remark}


By combining Theorem~\ref{thm:var_d}, Remark~\ref{remark:sum_bound} and Remark~\ref{remark:reverse_temperature} we have the following lemma.

\begin{lemma}

Let the type distribution $D$ be a MRF with inverse temperature $\beta<1$.

Then:

\begin{align*}
    Var[v(\vT,C(\vT)] \leq \frac{2(\srev)(\core)}{1-\beta} 
\end{align*}
\end{lemma}
}













==> MRF/tree.tex <==
\section{Tree Structured MRFs}\label{subsec:core_trees}

In this section, we consider the special case where the MRF is defined on a tree. We design a greedy algorithm (Algorithm~\ref{algo:min_norm}) to efficiently decide whether there exists a metric $d$ from a parametrized family of metrics, such that the corresponding $d$-Dobrushin interdependent matrix has infinity norm less than $1$. Note that the existence of such a metric $d$ implies that $\rho_d(\vT)<1$. See Appendix~\ref{sec:appx_tree_MRF_alg} for the description of Algorithm~\ref{algo:min_norm} and its analysis.   

Inspired by Algorithm~\ref{algo:min_norm}, we also provide the following sufficient condition for the spectral radius $\rho_d(\vT)$ to be less than $1$. Note that our condition contains high temperature regime and goes beyond that.

\begin{lemma}\label{lemma:tree_sufficient_condition}
Given a MRF $\vT$ defined over a tree $G(V,E)$, if there exists a set of parameter $\{w_e\}_{e\in E}\in \mathbb{R}_+$, such that 
 $$k(\vT)=\max_{u\in V} w_{(p(u),u)} \beta_{p(u),u} + \sum_{c \in C(u)}\frac{\beta_{u,c}}{w_{(u,c)}},$$ where $p(u)$ is the parent of $u$ and $C(u)$ is the set of children of $u$, then there exists a metric $d(\cdot,\cdot)$ so that $\rho_d(t)\leq k(\vT)$.
 
If we set $w_e=1$ for all edges $e$,
then $k(\vT)=\beta(\vT)$.

If we consider the case where $G=(V,E)$ a tree where each node has at most $b$ children and for each $(u,v)\in E$, $\beta_{u,v} < \frac{1}{2\sqrt{b}}$,
then by choosing $w_e=\sqrt{b}$ for each edge $e\in E$, the condition holds for each node $u\in V$:
\begin{align*}
    \sqrt{b}\beta_{u,p} + \frac{1}{\sqrt{b}} \sum_{c \in C(u)}\beta_{u,c} < 1
\end{align*}

Note that $\beta(\vT)$ may be higher than $\frac{\sqrt{b}}{2}$ violating the Dobrushin uniqueness condition. 
\end{lemma}

\begin{corollary}
%Let the type distribution $D$ be a MRF such that the corresponding graph is a complete $d$-ary tree and the value of the Markov influence between any pair of items is bounded by $\beta < \frac{1}{2\sqrt{d}}$.
Let MRF $\vT$ be defined on a tree $G=(V,E)$ where each node has at most $b$ children and for each $(u,v)\in E$, $\beta_{u,v} < \beta^*< \frac{1}{2\sqrt{b}}$, then $\Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1- 2\sqrt{d}\beta^*} $.
\end{corollary}


The new sufficient condition allows us to apply Theorem~\ref{thm:XOS} to a broader regime of parameters when the MRF is defined on a tree, e.g., complete $b$-ary trees with pairwise Markov influece $\beta_{i,j}$ as high as $\frac{1}{2\sqrt{b}}-\varepsilon$, which is not in the high temperature regime.%is that when the MRF is defined on a tree, 


\subsection{Details about the Tree Structured MRF}\label{sec:appx_tree_MRF_alg}
Assume the MRF is defined over a tree $G=(V,E)$ with only pair-wise potentials (that means that $G$ is a simple graph).
We need some additional notation.
Assume $G(V,E)$ is a tree.
For any item $u\in V$,
we denote by $C(u)$ the set of items that are children of $u$ in $G$.
Moreover when we refer to the father of item $u$,
we mean the item that is the father of item $u$ in the graph that the MRF is defined.
Similarly when we refer to the neighbors of an item $u$,
we mean its children and its parent.
In a high level idea,
the purpose of this section is to identify a metric function $d$ w.r.t. $\cup_{i\in[n]}T_i$ that minimizes the infinity norm of the $d$-Dobrushin interdependent matrix $A$ (as presented in Lemma~\ref{thm:var_d}),
so that we can effectively bound the variance of function $v(\vT,C(\vT))$.

First we need the following change in notation.
We consider the set $\E = \cup_{i \in [n]} \{(t_i,i) : t_i \in T_i\}$,
and we say that an $\vT^{\E} \in \E^n$ is valid if for each $i\in [n]$, $t_i^{\E}=(t_j,k)$ then $t_j \in T_i$ and $k=i$.
From now on,
when we refer to set $\E^n$,
we mean the subset of $\E^n$ that consists of valid elements.
We consider the following bijection mapping between $\bm{T}$ and $\E^n$: $\bm{t} \in T$ is mapped to $\bm{t}^{\E} \in \E^n$ such that $t_i^{\E} = (t_i,i)$.
We consider the MRF $D^{\E}$,
that first samples $\bm{t}\sim D$ and outputs $\bm{t}^{\E}$,
note that the structural information of the MRF $D^{\E}$ and $D$ are the same.
Similarly we define $g^{\E}(\bm{t}^{\E}):\E^n \rightarrow \mathbb{R}$ such that $g^{\E}(\bm{t}^{\E}) = v(\vT,C(\vT))$.



We need to introduce the following parameters.
Let $A^{TV}=\{\alpha^{TV}_{i,j}\}_{i,j\in[n]}$ be the $d$-Dobrushin interdependent matrix of $D$ under the trivial metric $d(t_i,t_i')=\mathds{1}_{t_i \neq t_i'}$,
that means:

\begin{align*}
    \alpha^{TV}_{i,j} =  \sup_{\substack{t_{-i},t'_{-i} \in T_{-i}, \\ t_{-i-j}, = t'_{-i-j}, t_j \neq t'_j} } d_{TV}\left(D_{i\mid t_{-i}}, D_{i\mid t_{-i}'} \right)
\end{align*}

We consider the following metric $d: \E \times \E \rightarrow \mathbb{R}$ parametrized by $v_i>0$, for $i\in[n]$:

\begin{align}
    d\left( (t_i,i), (t_i',i') \right) = 
    \begin{cases}
    v_i \mathds{1}_{t_i \neq t_i'} \quad & \text{if $i=i'$} \\
    \max_{k\in [n]}v_k \quad & \text{o.w.}
    \end{cases} \label{eq:param}
\end{align}


Note that $\alpha_{i,j}$ (as defined in Lemma~\ref{thm:var_d}) of the $d$-Dobrushin Interdependent matrix $A$ over MRF $D^{\E}$ satisfies:

\begin{align*}
    \alpha_{i,j} = & \sup_{\substack{t^{\E}_{-i},t'^{\E}_{-i} \in \E^n_{-i}, \\ t^{\E}_{-i-j}, = t'^{\E}_{-i-j}, t^{\E}_j \neq t'^{\E}_j} } \frac{W_{1,d}\left(D^{\E}_{i\mid t^{\E}_{-i}}, D^{\E}_{i\mid t'^{\E}_{-i}} \right)}{d\left((t_j,j),(t_j',j)\right)} \\
    = & \sup_{\substack{t_{-i},t'_{-i} \in T_{-i}, \\ t_{-i-j}, = t'_{-i-j}, t_j \neq t'_j} } \frac{v_i}{v_j} d_{TV}\left(D_{i\mid t_{-i}}, D_{i\mid t_{-i}'} \right) \\
    = & \frac{v_i}{v_j} \alpha^{TV}_{i,j}
\end{align*}

If $u$ is a child of $p$,
then we define $w_{(u,p)}=w_{(p,u)}= \frac{v_u}{v_p}$.
Therefore if $u$ is a child of $p$ we have that:

\begin{align*}
    \alpha_{u,p} = & w_{(u,p)} \alpha^{TV}_{u,p} \\
    \alpha_{p,u} = & \frac{1}{w_{(u,p)}} \alpha^{TV}_{p,u}
\end{align*}

%
%
%
\begin{remark}\label{remark:param}
Another way to define a metric $d$ parametrized as described in \eqref{eq:param},
is to provide a set of parameters $\{w_e\}_{e\in E}$,
where $w_{(u,p(u))}=\frac{v_u}{v_{p(u)}}$, where $p(u)$ is the parent of $u$.
Moreover the sum of the elements of the row that corresponds to item $u$ of the $d$-Dobrushin Interdependent matrix is equal to:
\begin{align*}
    w_{(u,p(u))} \alpha^{TV}_{u,p(u)} + \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}}
\end{align*}
\end{remark}
%
%
%
Now we are ready to describe how to choose the values of $w_{(u,v)}$ so that we minimize the infinity norm of the $d$-Dobrushin interdependent matrix $A$.
Assume that $k^*$ is the minimum value of the infinity norm of the $d$-Dorbushin interdependent matrix  $A$, where $d$ is parametrized as described in \eqref{eq:param}. We are going to provide a greedy algorithm,
that given a prediction $k$ about the value of $k^*$,
outputs if $k=k^*$,
if $k>k^*$ or if $k< k^*$.
The algorithm is presented in Algorithm~\ref{algo:min_norm}.


\begin{algorithm}[H] 
\caption{Given a MRF $D$ and over a tree $G(V,E)$, access to the $d$-Dobrushin interdependent matrix $A^{TV}=\{\alpha^{TV}_{i,j}\}_{i,j\in[n]}$ when $d$ is the trivial metric and a prediction $k$,
output whether $k$ is bigger, small or equal than the minimum infinity norm of the $d$-Dobrushin interdependent matrix $A$, where $d$ is parametrized as in equation~\eqref{eq:param}
}
\label{algo:min_norm}
 arbitrary root $G$ at item $r$
 $U\leftarrow V-\{r\}$ 
 $S\leftarrow \emptyset$ 
 \While{$ U \neq \emptyset$}{
  		$u \leftarrow \text{an item in $U$ such that all of its child are in $S$}$\;
  		\eIf{$k - \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} > 0$}{
   			$p \leftarrow \text{parent of $u$}$\;
   			$w_{(u,p)}\leftarrow \frac{1}{\alpha^{TV}_{u,p}} \left(k - \sum_{c \in C(u)} \frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} \right) $\;
   			$U \leftarrow U - \{u\}$\;
   			$S \leftarrow S \cup \{u\}$\;
   }
   {
       	Output that $k < k^*$\;
    }
  }

 	\uIf{$\sum_{c \in C(r)} \frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} = k $}{
 		Output that $k = k^*$\;
 	}
 	\uElseIf{$\sum_{c \in C(r)}\frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} > k $}{
 		Output that $k < k^*$\;
 	}
 	\Else{$\sum_{c \in C(r)}\frac{\alpha^{TV}_{r,c}}{w_{(r,c)}} < k $}{
 		 Output that $k > k^*$\;
 	}
 %\caption{Minimum $||A||_\infty$ value Comparator}
\end{algorithm}



Intuitively,
Algorithm~\ref{algo:min_norm} use the predicted value of $k$ and tries to construct a valid metric $d$ such that the sum of elements of each row of the $d$-Dobrushin Interdependence matrix $A$ is no more than $k$.
We keep two sets of items,
one set of Explored items (the set $S$),
such that for each item $u\in S$,
we have defined the parameter $w_{(u,p)}$,
where $p$ is the parent of $u$,
and one set of Unexplored items (the set $U$) that tracks the items $u\in U$ such that we have not defined the parameter $w_{(u,p)}$,
where $p$ is the parent of $u$. The algorithm starts by exploring the items that are located at the leaves of the tree. Once we have explored all the items,
except for the root $r$,
it suffices to verify that the sum of the elements of the row of $A$ that corresponds to the root is greater, less or equal to $k$.


\begin{lemma}
\label{lem:norm_estimation}
Given a MRF $D$ over a tree $G$ and let $k^*$ be the minimum infinite norm of the $d$-Dobrushin interdependence matrix $A$ where $d$ is a metric parametrized as in \eqref{eq:param}.
Given a prediction $k$,
Algorithm~\ref{algo:min_norm} outputs whether or not $k=k^*$, $k<k^*$ or $k>k^*$ in time $O(n)$. 
\end{lemma}

\begin{proof}
First we are going to prove that the running time of the algorithm is $O(n)$.
We note that we can identify a sequence of items $u_i$,
such that for each $i$,
all the children of $u_i$ are in $\{u_j\}_{1 \leq j<i}$,
just by performing a DFS on $G$ from the root $r$,
which takes time $O(n)$.
We note that we visit the items of $G$ in the While-loop,
in a sequence like the one described above.


We also note that each item is examined at most once in the While-loop,
and each time we examine an item,
we only need to access its neighbors.
Therefore the total running time of the algorithm is $O(n)$.




Now we are going to prove the correctness of the algorithm.
Our goal is to construct a metric $d$ parametrized as in \eqref{eq:param}.
By Remark~\ref{remark:param},
it is enough to define the parameters $\{w_e\}_{e\in E}$,
where $w_{(u,p(u))}= \frac{v_u}{v_{p(u)}}$,
where $p(u)$ is the father of $u$.
First we note that each time we define a parameter $w_{(u,v)}$,
we define the entries $\alpha_{u,v}$ and $\alpha_{v,u}$ of the $d$-Dobrushin interdependent matrix $A$.
The correctness of the algorithm is based on the following observation.
Suppose we have selected item $u$ in the first step of the While-loop,
whose father is $p$.
We assign $w_{(u,p)}$,
the maximum possible value,
such that the sum of the elements of the row that corresponds to item $u$ of matrix $A$ is $k$.
Now we note that the higher the value of $w_{(u,p)}$,
the smaller the value of $\alpha_{p,u}$.
Therefore,
for each pair of items $u,v$,
where $v\in C(u)$,
the algorithm assigns the smallest value of $\alpha_{u,v}$ over any $d'$-Dobrushin matrix $A'$,
where $d'$ is another metric parametrised by \eqref{eq:param} such that the sum of the elements of the row that corresponds to $u$ is at most $k$.
Therefore when the algorithm output that $k < k^*$ in the While-loop,
it means that there is not a metric $d'$ parametrized by \eqref{eq:param} so that the $d'$-Dobrushin matrix $A$,
has infinite norm at most $k$.



After the algorithm exits the While-loop,
it means that it has defined all parameters $w_{(u,v)}$ so that for each item $u\in V-\{r\}$,
the sum of the elements of the row that corresponds to $u$ in $A$ is equal to $k$.
We also know that for any metric $d'$ as parametrised in \eqref{eq:param},
that the $d'$-Dobrushin interdependent matrix $A'$,
such that $||A'||_\infty \leq k^*$,
has for any $v \in C(r)$ $\alpha_{r,v} \leq \alpha'_{r,v}$.



Let $k_r$ be the sum of the elements of the row of $A$ that corresponds to $r$.


If $k_r > k$,
then since $\alpha_{r,u} \leq \alpha'_{r,u}$,
where $A'$ is the $d'$-Dobrushin interdependent matrix of a metric $d'$ parametrised as in \eqref{eq:param},
implies that there does not exists a metric $d'$ parametrised as in \eqref{eq:param} such that infinite norm of the $d'$-Dobrushin interdependent matrix is at most $k$.


Similarly, if $k_r = k$,
then there does not exists a metric $d'$ parametrised as in \eqref{eq:param} such that $d'$-Dobrushin interdpendent matrix $A'$ has infinity norm less than $k$.
Therefore $k^* = k$.




Finally, if $k_r < k$,
then for sufficiently small $\epsilon>0$,
if we rerun the algorithm with prediction $k-\epsilon$ (conditioning on choosing the same root in the initialization of the algorithm),
then it is going to calculate another metric $d'$ and a $d'$-Dobrushin Interdependent matrix $A'$,
such that for each item $u \in V -\{r\}$,
the sum of the elements of the row of $A'$ that corresponds to $u$ is $k-\epsilon$,
and the sum of the elements of the row of $A'$ that corresponds to $r$ is $k_r + \delta(\epsilon)$,
where $\delta(\epsilon)>0$ and $\lim_{\epsilon \rightarrow 0}\delta(\epsilon) = 0$.
Therefore $k^* \leq ||A'||_\infty < k$.


\end{proof}


\notshow{
\argyrisnote{Argyris: Should I remove them? I don't think they add anything in terms of context.}

A corollary of Lemma~\ref{lem:norm_estimation} is the following.

\begin{corollary}\label{cor:algo_output}
We can verify in time $O(n)$ using Algorithm~\ref{algo:min_norm} with prediction $k=1$ if $k^* < 1$.

If $k^* < 1$,
then using binary search with Algorithm~\ref{algo:min_norm} $\log(\epsilon)$ times,
we can approximate the value of $k^*$ within an additive $\epsilon$ term. 
The total running time of this precudure is $O(n \log(\epsilon))$
\end{corollary}


Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:var_d} and Remark~\ref{remark:sum_bound} we obtain the following Theorem:

\begin{theorem}
\label{thm:metric_var}
Given a MRF $D$ over a tree $G$ with $n$ items,
let $k^*$ be the minimum infinite norm of the $d$-Dobrushin Interdependence matrix,
where $d$ us parametrized as in \eqref{eq:param}.
For any $\epsilon>0$,
such that $k^* < 1- \epsilon$,
we can identify a metric $d$ such that the $d$-Dobrushin interdpendent matrix $A$ satisfies $||A||_\infty \leq k^* + \epsilon$ in time $O(n \log(\epsilon))$.
If we can identify such a metric $d$,
then we also have:

\begin{align*}
    Var[v(\vT,C(\vT)] \leq \frac{2(\srev)(\core)}{1-k^*-\epsilon} 
\end{align*}
\end{theorem}


}



%\subsection{Buyers valuation is a MRF over a General Class of Trees}\label{subsec:core_d_trees}
\subsection{Proof of Lemma~\ref{lemma:tree_sufficient_condition}}\label{subsec:core_d_trees}
\begin{prevproof}{Lemma}{lemma:tree_sufficient_condition}
The proof of the lemma is directly inspired by Algorithm~\ref{algo:min_norm}.
Let $d$ be a metric parametrized as described in \eqref{eq:param},
then according to Remark~\ref{remark:param} it is enough to define parameters $\{w^*_e\}_{e\in E}$.
Let $A$ be the $d$-Dobrushin interdependent matrix of $\vT$,
under the metric $d$ we just described, where for each $e\in E$ we set $w^*_e = w_e$.
Let $A^{TV}=\{a^{TV}_{u,v}\}_{u,v\in V}$ be the $d$-Dobrushin interdependent matrix of $\vT$ under the trivial metric.
By Lemma~\ref{lemma:Dobruthin properties} we have that $\alpha^{TV}_{u,v} \leq \beta_{u,v}$.
Therefore the sum of elements of the row that corresponds to item $u$ of $A$ can be bounded by:
\begin{align*}
w_{(p(u),u)} \alpha^{TV}_{p(u),u} + \sum_{c \in C(u)}\frac{\alpha^{TV}_{u,c}}{w_{(u,c)}} \leq w_{(p(u),u)} \beta_{p(u),u} + \sum_{c \in C(u)}\frac{\beta_{u,c}}{w_{(u,c)}} \leq k(\vT)    
\end{align*}

The inequality above implies that the infinity norm of $A$ is upper bounded by $k(\vT)$.
Since the spectral radius of $A$ is upper bounded by the infinity norm of $A$,
we conclude that $\rho_d(\vT) \leq k(\vT)$.
\end{prevproof}

\notshow{
\argyrisnote{Argyris: I believe we should erase the rest of this section.}


In this section we are going to demonstrate how we can use Lemma~\ref{lem:norm_estimation} in order to provide a condition such that we can efficiently bound the covariance of $v(\vT,C(\vT))$,
when the buyers valuation is a MRF but does not satisfies the Dobrushin Uniqueness Condition.
We assume that the MRF $D$ is over a Tree and there exists a parameter $w\in \mathbb{R}_+$,
such that $k=\max_{\substack{u \in V,\\ \text{$p$ father of $u$}}}w \beta_{u,p} + \frac{1}{w}\sum_{c \in C(u)}\beta_{u,c} < 1$.
We are going to show that are instances of trees in this category where the inverse temperature of the MRF could be arbitrary large,
and violate the Dobrushin Uniqueness Condition.



We are going to prove that there exists a metric $d$, parametrized as in \eqref{eq:param} such that infinity norm of the $d$-Dobrushin Interdependent matrix is bounded by $k$ (This prediction is a generalization of \cite{levin2017markov}, Section~15.4, Theorem~15.6).




\begin{lemma} \label{lem:tree_metric}
Given a MRF $D$ over a tree $G(V,E)$ and a parameter $w\in \mathbb{R}_+$,
let $k=\max_{\substack{u \in V,\\ \text{$p$ father of $u$}}}w \beta_{u,p} + \frac{1}{w}\sum_{c \in C(u)}\beta_{u,c} < 1$,
then running Algorithm~\ref{algo:min_norm} with prediction $k$,
outputs that there exists a metric $d$ such that the infinite norm of the $d$-Dobrushin Interdependent matrix is bounded by $k$.
\end{lemma}
\yangnote{Why do we need to set $w$ to be the same for each edge? Why do we need the algorithm to prove this claim? It follows from the definition, no?}
\begin{proof}
First we assume that root of $G$ is the same as the root selected in Algorithm~\ref{algo:min_norm}.
We are going to prove by induction that between any pair of items $u,p$, where $p$ is the parent of $u$,
$w_{(u,p)}\geq w$ (this statement does not cover the case where $u$ is the root of the tree).


In order to prove the base case,
it is enough to prove that the induction hypothesis holds for the leafs of $G$.
Let $u$ be a leaf and $p$ its parent,
noting that $w \beta_{u,p} \leq k$,
the algorithm makes the following assignment:

\begin{align*}
    w_{(u,p)} \leftarrow \frac{k}{\beta_{u,p}} \geq w
\end{align*}

Therefore the base case is now settled.

For the induction step,
we assume that we visit an item $u$ such that for each $c \in C(u)$,
it holds that $w_{(u,c)} \geq  w$.
Let $p$ be the parent of $u$,
Algorithm~\ref{algo:min_norm} makes the following assignment:
\begin{align*}
    w_{(u,p)} \leftarrow & \frac{1} {\beta_{u,p}} \left( k - \sum_{c\in C(u)}\frac{\beta_{c,u}}{w_{c,u}} \right) \\
    \geq & \frac{1} {\beta_{u,p}} \left( k - \frac{1}{w}\sum_{c\in C(u)}\beta_{c,u} \right) \\
    \geq & \frac{1} {\beta_{u,p}}  w \beta_{u,p}  \\
    = & w
\end{align*}

The last inequality holds by the definition of $k$.
Therefore for any edge $(u,v)\in E$,
Algorithm~\ref{algo:min_norm} assignes $w_{(u,v)} \geq w$.
This fact implies that the Algorithm~\ref{algo:min_norm} does not output $k<k^*$ on the While-Loop.


Now we turn our attention to the root $r$.
It is enough now to verify that $\sum_{c \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} < k $,
which would imply that $k > k^*$ and we can conclude the proof.
Noting that $w_{(u,v)} \geq w$ for each $(u,v)\in E$:
\begin{align*}
    \sum_{c  \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} \leq \frac{1}{w}\sum_{c \in C(r)}\beta_{r,c}  \leq k
\end{align*}


\end{proof}


We make the following observation.

\begin{observation}\label{obs:specific_metrics}
If we apply Lemma~\ref{lem:tree_metric} with $w=1$,
then the value of $k$ is equal to the inverse temperature of $D$.


If we consider the case where $G(V,E)$ is the complete $d$-ary tree,
such that for each $(u,v)\in E$, $\beta_{u,v} \leq \beta < \frac{1}{2\sqrt{d}}$,
then for each node $u\in V$ it holds that:
\begin{align*}
    \sqrt{d}\beta_{u,p} + \frac{1}{\sqrt{d}} \sum_{c \in C(u)}\beta_{u,c} < 1
\end{align*}

Therefore we can apply Lemma~\ref{lem:tree_metric} on $D$ with parameter $w=\sqrt{d}$ and prediction $k=2\sqrt{d} \beta$.

We note that the inverse temperature in this case could be as high as $\frac{\sqrt{d}}{2}$ which would violate the Dobrushin condition.
\end{observation}


%Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:metric_var} and Observation~\ref{obs:specific_metrics} we obtain the following result.

}




\notshow{

In this section we are going to demonstrate how we can use Lemma~\ref{lem:norm_estimation} in order to provide a condition such that we can efficiently bound the covariance of $v(\vT,C(\vT))$,
when the buyers valuation is a MRF but does not satisfies the Dobrushin Uniqueness Condition.
We assume that the MRF $D$ is over a $d$-ary Tree where each pairwise-potential is bounded by $\beta\leq \frac{1}{2\sqrt{d}}$.
Note the inverse temperature of this MRF could be as high as $\frac{\sqrt{d}}{2}$,
which would violate the Dobrushin Uniqueness Condition.



We are going to prove that there exists a metric $d$, parametrized as in \eqref{eq:param} such that infinity norm of the $d$-Dobrushin Interdependent matrix is bounded by $2 \beta \sqrt{d}$ (This prediction is based on \cite{levin2017markov}, Section~15.4, Theorem~15.6).



\begin{lemma} \label{lem:tree_metric}
Given a MRF $D$ over a $d$-ary tree $G(V,E)$ such that the Markov influence between any pair of items is bounded by $\beta$,
then running Algorithm~\ref{algo:min_norm} with prediction $k=2\beta \sqrt{d}$,
conditioned on the fact that the root of $G$ is the same as the root selected in Algorithm~\ref{algo:min_norm},
outputs that there exists a metric $d$ such that the infinite norm of the $d$-Dobrushin Interdependent matrix is bounded by $2\beta \sqrt{d}$.
\end{lemma}

\begin{proof}
First we are going to prove by induction that between any pair of items $u,p$, where $p$ is the parent of $u$,
$w_{(u,p)}\geq \sqrt{d}$ (this statement does not cover the case where $u$ is the root the $d$-ary tree).


In order to prove the base case,
it is enough to prove that the induction hypothesis holds for the leafs of $G$
Let $u$ be a leaf and $p$ its parent,
the algorithm makes the following assignment:

\begin{align*}
    w_{(u,p)} \leftarrow \frac{2 \sqrt{d} \beta}{\beta_{u,v}} \geq 2 \sqrt{d}
\end{align*}

Therefore the base case is now settled.

For the induction step,
we assume that we visit an item $u$ such that for each $c \in C(u)$,
it holds that $w_{(u,c)} \geq  \sqrt{d}$.
Let $p$ be the parent of $u$,
Algorithm~\ref{algo:min_norm} makes the following assignment:
\begin{align*}
    w_{(u,p)} \leftarrow & \frac{1} {\beta_{u,p}} \left( 2 \beta \sqrt{d} - \sum_{c\in C(u)}\frac{\beta_{c,u}}{w_{c,u}} \right) \\
    \geq & \frac{1} {\beta} \left( 2 \beta \sqrt{d} - \sum_{c\in C(u)}\frac{\beta}{w_{c,u}} \right) \\
    \geq &  \left( 2 \sqrt{d} - \sum_{c\in C(u)}\frac{1}{\sqrt{d}} \right) \\
    = & \left( 2 \sqrt{d} - \frac{d}{\sqrt{d}} \right) = \sqrt{d}\\
\end{align*}

Therefore for any edge $(u,v)\in E$,
Algorithm~\ref{algo:min_norm} assignes $w_{(u,v)} \geq \sqrt{d}$.
This fact implies that the Algorithm~\ref{algo:min_norm} does not output $k<k^*$ on the While-Loop.


Now we turn our attention to the root $r$.
It is enough now to verify that $\sum_{c \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} < 2\beta \sqrt{d} $,
which would imply that $k > k^*$ and we can conclude the proof.
We note that according to the fact that $w_{(u,v)} \geq \sqrt{d}$ for each $(u,v)\in E$:
\begin{align*}
    \sum_{c  \in C(r)}\frac{\beta_{r,c}}{w_{r,c}} \leq \sum_{c \in C(r)}\frac{\beta}{\sqrt{d}}  = \sqrt{d} \beta < 2\sqrt{d}\beta
\end{align*}


\end{proof}



Combining Corollary~\ref{cor:algo_output}, with Theorem~\ref{thm:metric_var} and Lemma~\ref{lem:tree_metric} we obtain the following result.




\begin{lemma}

Let the type distribution $D$ be a MRF such that the corresponding graph is a complete $d$-ary tree and the value of the Markov influence between any pair of items is bounded by $\beta < \frac{1}{2\sqrt{d}}$.
Then:

\begin{align*}
    Var[v(\vT,C(\vT))] \leq \frac{2(\srev)(\core)}{1- 2\sqrt{d}\beta} 
\end{align*}
\end{lemma}

}

==> impossibility_copies_setting.tex <==
\subsection{Lower Bound for the Copies Setting}\label{sec:LB_copies}

We consider a valuation that is generated by a MRF $D$,
and we prove that the optimal revenue in the COPIES settings can be exponential in $\Delta(\vT)$, while both $\srev$ and $\brev$ are less than $2$. Indeed, we prove an even stronger result that the gap is exponential in the inverse temperature, which is an upper bound of $\Delta(\vT)$.


\argyrisnote{
\begin{theorem}\label{thm:COPIES_example}
For any value of $n\in \mathbb{N}$ and $\beta \in \mathbb{R}_+$
there exists an MRF $D$ with $n+1$ nodes and only pairwise potentials,
such that the Markov influence $\beta_{i,j}\leq \beta$ for every pair $i$, $j$ and it holds that the expected optimal revenue in the COPIES settings can be arbitrarily close to 
$\frac{1}{2}\exp(2\beta n)$,
while $\max\{\brev, \srev\} < 2$. Note that $\Delta(t)\leq \beta n$.
\end{theorem}
}

\begin{prevproof}{Theorem}{thm:COPIES_example}
We construct the MRF in the following way.
The first item has support $T_1=\{2^0,2^1,2^2,\ldots,2^{k^n-1}\}$,
where $k\in \mathbb{N}$ is going to be defined later.
Let $\epsilon_1,\ldots,\epsilon_k$ be some tiny values,
the support for the other items is $T_r=\{\epsilon_i\}_{i\in[k]}$.
We consider the following node potential for the first item:
\begin{align*}
    \psi_1(2^i) =
    \begin{cases}
    \ln(\frac{1}{2^{i+1}}) \quad &\text{if $0 \leq i \leq k^n-2$} \\
    \ln(\frac{1}{2^{i}}) & \text{if $i = k^n-1$}
    \end{cases}
\end{align*}

The node potentials for the other items is:

\begin{align*}
    \psi_i (a) =\ln\left(\frac{1}{\exp(\beta)+ (k-1)\exp(-\beta)}\right)
\end{align*}

for all $i\in[2,n+1]$ and $a\in T_r$.


Note that $|T_1|=k^n$ and $|T_r^n| = k^n$,
therefore for each $t_1 \in T_1$,
we can identify a unique $t_{-1} \in T_r^n$.
More formally we consider a bijective function $c: T_1 \rightarrow T_r^n$.


We define pair-wise potentials
between the first item and the $j$-th item:
%$\psi_{i,j}(\cdot, \cdot)$ between item $i$ and item $j$:

\begin{align*}
    \psi_{1,j}(t_1,t_j) =
    \begin{cases}
    \beta  &\text{if $t_j =c(t_1)_j$} \\
    -\beta  &\text{if $t_j \neq c(t_1)_j$} \\
    \end{cases}
\end{align*}

\argyrisnote{
(Maybe we should rewrite it as:)
We define pair-wise potentials
between the first item $t_i \in T_1$ and the $j$-th item $\epsilon_j \in T_r$:
%$\psi_{i,j}(\cdot, \cdot)$ between item $i$ and item $j$:
\begin{align*}
    \psi_{1,j}(t_1,\epsilon_j) =
    \begin{cases}
    \beta  &\text{if $\epsilon_j =c(t_1)_j$} \\
    -\beta  &\text{if $\epsilon_j \neq c(t_1)_j$} \\
    \end{cases}
\end{align*}
}

%\begin{align*}
%    \psi_{0,j}(t_0,t_j) =
%    \begin{cases}
%    0 \quad & \text{if $i,j \neq 0$} \\
%    \beta  &\text{if $i = 0$ and $t_j =c(t_i)_j$} \\
%    -\beta  &\text{if $i = 0$ and $t_j \neq c(t_i)_j$} \\
%    \end{cases}
%\end{align*}

{Let $Z$ be the normalizing constant so that the MRF with the potentials $\{\psi_i\}_{i \in[n+1]},\{\psi_{1,i}\}_{2 \leq i \leq n+1}$ mentioned above is a valid distribution.
That is $Z = \sum_{t \in \supp(D)} \prod_{i \in [n+1]}\exp(\psi_i(t_i)) \prod_{2 \leq i \leq n+1} \exp(\psi_{1,i}(t_1,t_i))$.}
For any $t_1 \in T_1$ we have that:

\begin{align*}
    \Pr_{t'\sim D}\left[t_1' = t_1 \land t_{-1}'= c(t_1) \right] = 
    &\frac{1}{Z}\exp(\psi_1(t_1)) \frac{\exp{(n \beta)}}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \\
\end{align*}
\begin{align*}
    &\Pr_{t'\sim D}\left[t_1' = t_1 \land t_{-1}' \neq c(t_1) \right] \\ =
    &\frac{1}{Z}\exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{\substack{t_{-1} \in T_{-1}:\\ t_{-1} \neq c(t_1)}} \prod_{i \in [2,n+1]} \exp\left(\psi_{1,i}(t_1, \{t_{-1}\}_i)\right) \\
    = & \frac{1}{Z}\exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{i \in [1,n]} {n \choose i} \left(k-1 \right)^i\left(\exp(-\beta) \right)^i \left(\exp(\beta)\right)^{n-i} \\
    = & \frac{1}{Z} \exp(\psi_1(t_1)) \frac{1}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \sum_{i \in [1,n]} {n \choose i} \left((k-1 )\exp(-\beta) \right)^i \left(\exp(\beta)\right)^{n-i} \\
    = & \frac{1}{Z} \exp(\psi_1(t_1)) \frac{(\exp(\beta)+(k-1)\exp(-\beta))^n - \exp(n \beta)}{(\exp(\beta)+(k-1)\exp(-\beta))^n} 
\end{align*}

Thus for any $t_1 \in T_1$, the marginal probability:

\begin{align*}
    f_1(t_1) = \frac{1}{Z} \exp(\psi_1 (t_1))
\end{align*}

{Note that $Z = \sum_{t_1 \in T_1} \exp(\psi_1(t_1)) = \sum_{i=0}^{k^n-2}\frac{1}{2^{i+1}} + \frac{1}{2^{k^n-1}}= 1$. Thus $f_1(t_1) = \exp(\psi_1(t_1))$.}
Therefore the marginal distribution of the first item is an Equal Revenue Distribution, which means that the revenue of any posted price mechanism for the first item, cannot be more than $1$.
Moreover, if we set $\max_{t_r \in T_r} \leq \frac{1}{2n}$,
then any posted price mechanisms for the rest $n$ items has revenue less or equal than $\frac{1}{2}$.
Thus $\srev < 2$.



Now we consider the following Mechanism in the copies settings.
We first collect the values for all the items but the first $\vT_{-1}$.
Then we let the first buyer to decide if she wants to buy the item at price $c^{-1}(t_{-1})$. This is similar to Ronen's lookahead auction~\cite{Ronen_2001}.
A lower bound on the revenue of this mechanism in the COPIES settings is:

\begin{align*}
    \sum_{t_1 \in T_1} t_1 \Pr_{t' \sim D} \left[ c^{-1}(t_{-1}) = t_1 \land t_1' =t_1 \right]
    = & \sum_{t_1 \in T_1} t_1 \exp(\psi_1(t_1)) \frac{\exp{(n \beta)}}{(\exp(\beta)+(k-1)\exp(-\beta))^n} \\
    = & \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n\sum_{t_1 \in T_1} t_1 \exp(\psi_1(t_1))  \\
    \geq & \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n\sum_{t_1 \in T_1}\frac{1}{2}  \\
    = & \frac{1}{2} \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n|T_1| \\
    = & \frac{1}{2} \left(\frac{1}{1 + (k-1)\exp(-2\beta)} \right)^n k^n \\
    = & \frac{1}{2} \left(\frac{k}{1 + (k-1)\exp(-2\beta)} \right)^n 
\end{align*}


Where the last inequality comes from $t_1\cdot \exp(\psi_1(t_1))  \geq \frac{1}{2}$.

Note that if we fix $\beta$ and let $k \rightarrow \infty$,
then $\lim_{k\rightarrow \infty}\left(\frac{k}{1 +(k-1)\exp(-2\beta)}\right)^n= \exp(2\beta n)$.

Therefore as $k\rightarrow \infty$,
the lower bound of the revenue of the proposed mechanisms becomes $\frac{\exp(2\beta n)}{2}$.
{Since we assumed that the value of the agent for each item except the first is less or equal than $\frac{1}{2n}$,
then the value of the agent for all but the first item is less or equal than $\frac{1}{2}$.
This implies that if the agent buys the whole bundle at price $p$,
then she also buys the first item at price $p-\frac{1}{2}$.
Let $\rev_1$ be the revenue of the posted price mechanism on the first item.
Since the marginal of the fist item is the Equal Revenue Distribution,
then $\rev_1\leq 1$.
Moreover by the argument described above,
we have that $\brev \leq \rev_1 + \frac{1}{2} < 2$.
Thus $\max(\srev, \brev) < 2$}.
\end{prevproof}


==> impossibility_dobrushin.tex <==
\subsection{Impossibility of Multiplicative Approximation under the Dobrushin Uniqueness Condition}\label{sec:inapprox_Dobrushin}
In this section, we show that there exist MRFs that satisfy the Dobrushin uniqueness condition, while $\srev$ and $\brev$ cannot guarantee any multiplicative approximation of the optimal revenue.





First we present the main building block of our construction.


\begin{lemma}
\label{lemma:mix_dobrushin}
Let $D'$ be a correlated valuation distribution over $2$ items with $\alpha(\vT)=\alpha$.
Let $D$ be a product distribution that has the same marginal distributions as $D'$.
Then for any $0\leq \alpha' \leq 1$,
we consider the distribution $D''$ that takes a sample from $D'$ with probability $\alpha'$ and takes a sample from $D$ with probability $1-\alpha'$.
Distribution $D''$ can be modeled as a MRF with finite inverse temperature
{such that $\Delta = \beta(\vT) \leq |\log((1-\alpha) p^2)|$,
where $p = \inf_{\vT \in \supp(D')} \Pr_{\vT' \sim D'}[\vT'=\vT]$}%$(\beta(\vT) < +\infty)$
and $\alpha(\vT) = \alpha' \cdot \alpha$.
Furthermore, $D''$ has the same marginal distribution as $D$ and $\rev(D'') \geq \alpha'\rev(D')$.
\end{lemma}


\begin{proof}
Assume that $D=D_1\times D_2$, where $D_1$ and $D_2$ are the marginals of  $D'$.% = (D_1',D_2')$ and $D^{''}=(D_1^{''},D_2^{''})$.
Let $T_i = \supp(D_i)$%=\supp(D_i')=\supp(D_i'')$
and $T= T_1 \times T_2$.
Let $A^{D'}=\{\alpha_{i,j}^{D'}\}_{i,j\in[2]}$ be the $d$-Dobrushin interdependent matrix of $D'$ and $A^{D''}=\{\alpha_{i,j}^{D''}\}_{i,j\in[2]}$ be the $d$-Dobrushin interdependent matrix of $D''$,
under the trivial metric.
Note that the diagonal entries of $A^{D'}$ and of $A^{D''}$ are zero.
%We denote by $I_{j \rightarrow i}^D$  the influence from random variable $D_i$ to random variable $D_j$.
%Similarly we denote by $I_{j \rightarrow i}^{D''}$ the influence from random variable $D_i''$ to random variable $D_j''$.
We have that:

\begin{align*}
\alpha_{i,j}^{D''}
= & \max_{  \substack{ t_j,t'_j \in T_j } }  
	%
	d_{TV} \left( D''_{i \mid t_j},
	D''_{i \mid t_j'}\right) \\
    = &\alpha' \max_{ t_j,t'_j \in T_j  }  
	%
	d_{TV} \left( D'_{i \mid t_j},
	D'_{i \mid t_j'}\right) \\
	=& \alpha' \alpha_{i,j}^{D'}
\end{align*}

In the statement of the lemma,
we assumed that $\alpha = ||A^{D'}||_\infty=\max(\alpha^{D'}_{1,2},\alpha^{D'}_{2,1})$.
We can easily infer the following.

\begin{align*}
    ||A^{D''}||_\infty = \max(\alpha_{1,2}^{D''},\alpha_{2,1}^{D''}) = \alpha' \max(\alpha_{1,2}^{D'},\alpha_{2,1}^{D'}) = \alpha' \cdot \alpha
\end{align*}

This concludes the fact that $D''$ has $\alpha(\vT) =\alpha' \cdot \alpha$.


Now we prove that $D''$ can be modeled as a MRF with finite inverse temperature.
We consider an MRF with potential functions $\psi_1(t_1) = 1,\forall t_1 \in T_1$, $\psi_2(t_2) = 1,\forall t_2 \in T_2$ and $\psi_{1,2}(\vT) = \ln\left( \Pr_{\vT' \sim D''}(\vT' =\vT)\right)$. Since Distribution $D''$ samples from the product distribution $D$ with probability $1-\alpha$,
we have that for each $\vT \in T$, {$\Pr_{\vT' \sim D''}(\vT' =\vT) \geq  (1-\alpha)p^2$. This is true because with probability $1-\alpha$ we sample from the product distribution $D''$,
and with probability at least $p^2$ we sample the type $\vT$.},
therefore the MRF we just described has finite inverse temperature {and $\Delta = \beta(\vT) = \max_{\vT \in \supp(D')} |\log\left(\Pr_{\vT' \sim D'}[\vT'=\vT] \right)|\leq |\log\left((1-\alpha)p^2 \right)|$}. In the case where the distribution is over two items, $\beta(\vT)= \max_{\vT \in T} |\psi_{1,2}(\vT)|$.
Moreover we can easily verify that the MRF we just described has the same joint distribution as $D''$.
Therefore $D''$ can be modeled as an MRF with finite inverse temperature.


We now prove that $\rev(D'') \geq \alpha' \rev(D')$.
This is true because we can simply use the optimal mechanism that induces $\rev(D')$ on $D''$.
Since $D''$ take a sample from $D'$ with probability $\alpha'$,
we are guaranteed that this mechanism has revenue at least $\alpha'\rev(D')$ on $D''$.

The fact that $D''$ has the same marginal distributions as $D'$ follows from the sampling procedure.
\end{proof}


Now we present an important result from \cite{HARTN_2019}.

\begin{lemma}[Theorem~A from \cite{HARTN_2019}]
\label{lemma:bad_distribution}
For any positive real number $N$, there exists a two item correlated distribution $D$,
such that for an additive buyer whose type is sampled from $D$, $\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}>N$.
%$\brev(D)=O(1)$ and $\srev(D) = O(1)$, while $\rev(D)>N$.
\end{lemma}

Now we are ready to present the  inapproximability result.

\argyrisnote{
(Maybe we should only state here the theorem and not before?)
\begin{theorem}\label{lem:inaprx_dob}
For any positive real number $N$ and any choice of $0< \alpha < 1$,
there exists a type distribution over $2$ items generated by a MRF $D$ with $\alpha(\vT) = \alpha$ and finite inverse temperature,
such that for an additive buyer whose type is sampled from $D$,
$\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}>\frac{\alpha}{2}\cdot N$.
\end{theorem}

}


\begin{prevproof}{Theorem}{lem:inaprx_dob}
Let $D'$ be the distribution over two items that is guaranteed to exist by Lemma~\ref{lemma:bad_distribution}. Since $D'$ is a two dimensional distribution, its Dobrushin coefficient is at most $1$.


Apply Lemma~\ref{lemma:mix_dobrushin} to $D'$ with parameter $\alpha'=\alpha$ to create another distribution $D$ which has the same marginals as $D'$ but with a Dobrushin coefficient at most $\alpha$. Moreover, $D$ can be expressed as an MRF with finite inverse temperature. Clearly, $\rev(D)\geq \alpha\cdot \rev(D')$, as one can simply achieve the LFS \argyrisnote{(I think it is RHS instead of LFS?)} using the optimal mechanism designed for $D'$. Also, $\srev(D')=\srev(D)$ as the two distributions have the same marginals. Finally, $\brev(D')\leq 2\srev(D')$. Suppose $b$ is the optimal price for the bundle, then we can set the two items separately each at price $b/2$. Clearly, whenever the bundle is sold, at least one item is sold. To conclude, $$\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}\geq \frac{\rev(D)}{2\srev(D)}\geq \frac{\alpha\cdot\rev(D')}{2\srev(D')}>\frac{\alpha}{2}\cdot N.$$
%we can generate a type distribution generated by a MRF $D'$ such that $\alpha(\vT) \leq \alpha$, has finite inverse temperature and has the same marginal distributions as $D$. Since the $\rev(D)$ can be arbitrary high, for a fixed value of $\alpha$ we can also make sure that $\rev(D') \geq \alpha\rev(D)$ is also arbitrary high.


%Since we assume that the agent has additive valuation, $\bm{SRev}(D')$ only depends on the marginal distribution of $D'$. Therefore since $D$ and $D'$ have the same marginal distributions,
%$\bm{SRev}(D')=\bm{SRev}(D)=O(1)$. We now prove that $\bm{BRev}(D') \leq 2\bm{SRev}(D)= O(1)$. Suppose $B$ is the posted price on the grand bundle. If we sell each item separately at price $B/2$, then we have revenue at least $\bm{BRev}/2$,so $\bm{SRev} \geq \bm{BRev}/2$. Therefore $\bm{SRev}=\bm{BRev}=O(1)$. This concludes our proof.
\end{prevproof}



%Lemma~\ref{lem:inaprx_dob} implies that even if we consider buyers type valuation that are generated by a MRF that satisfy the Dobrushin Uniqueness Condition, the revenue of simple mechanisms cannot be bounded by a multiplicative or additive term that depends on the value of $\alpha(\vT)$. A valid multiplicative or approximation bound should also include other parameters of the problem (like the inverse temperature).









==> improved_tail_bound.tex <==

\begin{lemma} \label{lemma:Dobrushin_tv}
Let $\vT=\{t_i\}_{i\in[n]}$ be a random variable generated by a distribution with Dobrushin coefficient $\alpha$.
For any $i$, $\EE\subseteq T_i$ and $t_{-i}\in T_{-i}$:

\begin{align*}
Pr_{t'' \sim D}\left[ t_i'' \in \EE \mid t_{-i}'' = t_{-i} \right] - \alpha 
\leq \Pr_{t'' \sim D}\left[ t_i'' \in \EE\right]
\leq \Pr_{t'' \sim D}\left[ t_i'' \in \EE \mid t_{-i}'' = t_{-i} \right] + \alpha
\end{align*}

\end{lemma}


\begin{proof}
We only prove that $\Pr_{t' \sim D}\left[ t_i' \in \EE\right]
\leq \Pr_{t' \sim D}\left[ t_i' \in \EE \mid t_{-i}' = t_{-i} \right] + \alpha$.
The other bound can be proved similarly.
W.l.o.g we assume that $i=n$.
For any $t_{-n}'\in T_{-n}$,
let $t_{-n}^k \in T_{-n}$ have the first $k$ coordinates the same as $t_{-n}'$ and the have the rest $n-1-k$ coordinates the same as $t_{-n}$.
Note that $t_{-n}^0=t_{-n}$ and $t_{-n}^{n-1}=t_{-n}'$
By the definition of influence we have that:

\begin{align*}
&\left| \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k-1} \right] - \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k} \right] \right| \leq I_{k \rightarrow n} \\
\Rightarrow  &  \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k-1} \right] - \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k} \right] \leq I_{k \rightarrow n}
\end{align*}

Thus we have that:
%
\begin{align*}
& \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n} \right] - \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}' \right] \\
= &  \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^0 \right] - \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{n-1} \right]  
\\
= & \sum_{k =1}^{n-1} \left(\Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k-1} \right] - \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}^{k} \right]\right)  
\\
\leq & \sum_{k=1}^{n-1}  I_{k \rightarrow n} \leq \alpha
\end{align*}

Therefore for any $t_{-n},t_{-n}' \in T_{-n}$ we have that  $Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n} \right] \leq \Pr_{t'' \sim D} \left[ t_n'' \in \EE \mid t_{-n}''=t_{-n}' \right] + \alpha$.



Fixing an event $t_{-n} \in T_{-n}$ and using the Law of Total Probability we have that:

\begin{align*}
\Pr_{t_n'' \sim D_n}\left[t_n'' \in \EE \right] 
=& \sum_{t_{-n}' \in T_{-n}} \Pr_{\vT'' \sim D}\left[ t_n'' \in \EE \mid t_{-n}''= t_{-n}' \right] \cdot f(\vT_{-n}') \\
 \leq & \sum_{t_{-n}' \in T_{-n}}\left( \Pr_{\vT'' \sim D}\left[ t_n'' \in \EE \mid t_{-n}''= t_{-n} \right] + \alpha \right) \cdot f(\vT_{-n}') \\
 = &  \Pr_{\vT'' \sim D}\left[ t_n'' \in \EE \mid t_{-n}''= t_{-n} \right] + \alpha 
\end{align*}


\end{proof}






\begin{lemma}
\label{lemma:Dobrushin_t_sum}
Let $D$ be a distribution with Dobrushin coefficient $\alpha$.
For an item $i$, set $\EE_{-i}\subseteq T_{-i}$,
let $\{a_{t_i}\}_{t_i \in T_i}$ be parameters such that for any $t_i \in T_i$:
%
\begin{align*}
    \Pr_{\vT'' \sim D}[t_i''=t_i \land t_{-i}'' \in \EE_{-i} ] = (f_i(t_i)+\alpha_{t_i}) \Pr_{t_{-i}'' \sim D_{-i}}[ t_{-i}'' \in \EE_{-i}]
\end{align*}
%
Then:
%
\begin{align*}
    \sum_{t_i \in T_i} \max(0,a_{t_i}) \leq \alpha
\end{align*}

\end{lemma}




\begin{proof}

We define the set $\EE_i=\{t_i \in T_i : a_{t_i}>0\}$.
First we have that:
%
\begin{align}
    \Pr_{t'' \sim D}[ t_i'' \in \EE_i \land t_{-i}'' \in \EE_{-i}]   
    = &  \sum_{\substack{t_i \in \EE_i}} \Pr_{\vT'' \sim D}[ t_i'' = t_i  \land t_{-i}'' \in \EE_{-i}]      \nonumber \\ 
    = & \sum_{\substack{t_i \in \EE''}} (f_i(t_i)+a_{t_i})  \Pr_{\vT''_{-i} \sim D_{-i}}[ t_{-i}'' \in \EE_{-i}]  \nonumber \\
    = &
    \Pr_{t_i'' \sim D_i}[t_i'' \in \EE_i]  \Pr_{\vT_{-i}'' \sim D_{-i}}[ t_{-i}'' \in \EE_{-i}]
    +
    \sum_{\substack{t_i \in \EE_i}} a_{t_i}  \Pr_{\vT_{-i}'' \sim D_{-i}}[ t_{-i}'' \in \EE_{-i}] \label{eq:bound}
\end{align}
%
%
Applying Lemma~\ref{lemma:Dobrushin_tv} on set  $\EE_i \subseteq T_i$:
%
%
\begin{align}
    \Pr_{\vT'' \sim D}[t_i'' \in \EE_i \land \vT_{-i}'' \in \EE_{-i}]    
    = & \sum_{\substack{\vT_{-i} \in \EE_{-i} }} \Pr_{\vT'' \sim D}[t_i'' \in \EE_i \mid t_{-i}''= t_{-i}] f_{-i}(\vT_{-i}) \nonumber \\
    \leq & \sum_{\substack{\vT_{-i} \in \EE_{-i} }} \left( \Pr_{\vT_i'' \sim D_i}[t_i'' \in \EE_i] + \alpha \right) f_{-i}(\vT_{-i}) \nonumber \\
    = &  \Pr_{\vT_i'' \sim D_i}[t_i'' \in \EE_i] \sum_{\substack{\vT_{-i} \in \EE_{-i} }} f_{-i}(\vT_{-i}) + \alpha \sum_{\substack{\vT_{-i} \in \EE_{-i} }}  f_{-i}(\vT_{-i}) \nonumber \\
    = &  \Pr_{\vT_i'' \sim D_i}[t_i'' \in \EE_{i}] \Pr_{\vT_{-i}'' \sim D_{-i}}[ t_{-i}'' \in \EE_{-i} ]+ \alpha \Pr_{\vT_{-i}'' \sim D_{-i}}[ t_{-i}'' \in \EE_{-i}] \label{eq:upper}
\end{align}

Since equation \eqref{eq:upper} is an upper bound on \eqref{eq:bound},
we can infer that:


\begin{align*}
    \sum_{t_i\in T_i} \max(a_{t_i}, 0) = \sum_{\substack{t_i \in \EE_i}} a_{t_i}  \leq  \alpha
\end{align*}

\end{proof}





\notshow{
\begin{lemma}
\label{lemma:Dobrushin_t_sum}
Let $D$ be a distribution with Dobrushin coefficient $\alpha$.
For an item $i$, set $\EE\subseteq T_i$, set $\EE'\subseteq T_{-i}$,
let $\{a_{t_i}\}_{t_i \in \EE}$ be parameters such that:
%
\begin{align*}
    \Pr_{\vT' \sim D}[t_i'=t_i \land t_{-i}' \in \EE' ] = (f_i(t_i)+\alpha_{t_i}) \Pr_{t_{-i} \sim D_{-i}}[ t_{-i} \in \EE']
\end{align*}
%
Then:
%
\begin{align*}
    \sum_{t_i \in \EE} \max(0,a_{t_i}) \leq \alpha
\end{align*}

\end{lemma}




\begin{proof}

We define the set $\EE''=\{t_i \in \EE : a_{t_i}>0\}$.
First we have that:

\begin{align}
    \Pr_{t \sim D}[ t_i \in \EE'' \land t_{-i} \in \EE']   
    = &  \sum_{\substack{t_i \in \EE''}} \Pr_{\vT' \sim D}[ t_i' = t_i  \land t_{-i}' \in \EE']      \nonumber \\ 
    = & \sum_{\substack{t_i \in \EE''}} (f_i(t_i)+a_{t_i})  \Pr_{\vT'_{-i} \sim D_{-i}}[ t_{-i}' \in \EE']  \nonumber \\
    = &
    \Pr_{t_i \sim D_i}[t_i \in \EE'']  \Pr_{\vT_{-i} \sim D_{-i}}[ t_{-i} \in \EE']
    +
    \sum_{\substack{t_i \in \EE''}} a_{t_i}  \Pr_{\vT_{-i} \sim D_{-i}}[ t_{-i} \in \EE'] \label{eq:bound}
\end{align}
%
%
By Lemma~\ref{lemma:Dobrushin_tv} on set  $\EE'' \subseteq T_i$:
%
%
\begin{align}
    \Pr_{\vT \sim D}[t_i \in \EE'' \land \vT_{-i} \in \EE']    
    = & \sum_{\substack{\vT_{-i} \in \EE' }} \Pr_{\vT' \sim D}[t_i' \in \EE'' \mid t_{-i}'= t_{-i}] f_{-i}(\vT_{-i}) \nonumber \\
    \leq & \sum_{\substack{\vT_{-i} \in \EE' }} \left( \Pr_{\vT_i \sim D_i}[t_i \in \EE''] + \alpha \right) f_{-i}(\vT_{-i}) \nonumber \\
    = &  \Pr_{\vT_i \sim D_i}[t_i \in \EE''] \sum_{\substack{\vT_{-i} \in \EE' }} f_{-i}(\vT_{-i}) + \alpha \sum_{\substack{\vT_{-i} \in \EE' }}  f_{-i}(\vT_{-i}) \nonumber \\
    = &  \Pr_{\vT_i \sim D_i}[t_i \in \EE''] \Pr_{\vT_{-i} \in T_{-i}}[ t_{-i} \in \EE' ]+ \alpha \Pr_{\vT_{-i} \in T_{-i}}[ t_{-i} \in \EE'] \label{eq:upper}
\end{align}

Since equation \eqref{eq:upper} is an upper bound on \eqref{eq:bound},
we can infer that:


\begin{align*}
    \sum_{t_i\in \EE} \max(a_{t_i}, 0) = \sum_{\substack{t_i \in \EE''}} a_{t_i}  \leq  \alpha
\end{align*}

\end{proof}
}





\begin{lemma}
$(\tail) \leq r (1 + n \alpha) $
\end{lemma}


\begin{proof}

For each buyer $i$ and $t_i \in T_i$, we consider the set $\EE_{i,t_i}= \{ t_{-i} \in T_{-i}: (t_i,t_{-i}) \notin R_i \}$ and parameters $\{a_{i,t_i}\}_{i \in[n], t_i \in T_i}$ such that:

\begin{align*}
    \Pr_{t'' \sim D}\left[t_i'' = t_i \land t_{-i}'' \in \EE_{i,t_i}\right] = (f(t_i) + a_{i,t_i})Pr_{t'' \sim D}\left[t_{-i}'' \in \EE_{i,t_i}\right]
\end{align*}

Using Lemma~~\ref{lemma:Dobrushin_t_sum} we have that:

\begin{align*}
      (\tail) = & \sum_{i \in [n]} \sum_{t_i > r} \Pr_{t'' \sim D}\left[ t_i'' = t_i \land t_{-i}'' \in \EE_{i,t_i}\right]  \cdot t_i \\
      = &
      \sum_{i \in [n]} \sum_{t_i > r} (f(t_i) + a_{i,t_i})Pr_{t'' \sim D}\left[ t_{-i}'' \in \EE_{i,t_i}\right]  \cdot t_i \\
      \leq &
      \sum_{i \in [n]} \sum_{t_i > r} f(t_i)Pr_{t'' \sim D}\left[ t_{-i} \in \EE_{i,t_i}\right]  \cdot t_i +
     \sum_{i \in [n]} \sum_{t_i > r} \alpha_{i,t_i} \Pr_{t \sim D}\left[ t_{-i} \in \EE_{i,t_i}\right]  \cdot t_i 
      \\
      \leq &
      \sum_{i \in [n]} \sum_{t_i > r} f(t_i)Pr_{t'' \sim D}\left[ t_{-i} \in \EE_{i,t_i}\right]  \cdot t_i +
      \alpha \sum_{i \in [n]} \Pr_{t \sim D}\left[ t_{-i} \in \EE_{i,t_i}\right]  \cdot t_i 
\end{align*}

We can think of $Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i$ as the expected revenue of the mechanisms that postes Price $t_i$ on all items except the $i$-th item, but allows the buyer to get only one item.
Therefore $Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i\leq r$.
This implies:

\begin{align*}
      (\tail)
      \leq &
      \sum_{i \in [n]} \sum_{t_i > r} f(t_i)Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i +
      \alpha \sum_{i \in [n]} \Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i \\
    \leq &
    \sum_{i \in [n]} \sum_{t_i > r} f(t_i)r +
      n \alpha r \\
    \leq &
    \sum_{i \in [n]} \Pr_{t_i \sim D_i}[t_i > r] r +
      n \alpha r \\
    \leq & r (1 + n \alpha)
\end{align*}

\end{proof}





\begin{lemma}
$(\tail) \leq r (1 + n \alpha) $
\end{lemma}


\begin{proof}

We consider the sets $\EE_{i,t_i}= \{ t_{-i} \in T_{-i}: (t_i,t_{-i}) \notin R_i \}$ and parameters $a_{t_i}$ such that:

\begin{align*}
    \Pr_{t' \sim D}(t_i' = t_i \land t_{-i}' \in \EE_{i,t_i}) = (f(t_i) + a_{t_i})Pr_{t \sim D}(t_{-i} \in \EE_{i,t_i})
\end{align*}

Using Lemma~~\ref{lemma:Dobrushin_t_sum} we have that:

\begin{align*}
      (\tail) = & \sum_{i \in [n]} \sum_{t_i > r} \Pr_{t' \sim D}(t_i' = t_i \land t_{-i}' \in \EE_{i,t_i})  \cdot t_i \\
      = &
      \sum_{i \in [n]} \sum_{t_i > r} (f(t_i) + a_{t_i})Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i \\
      \leq &
      \sum_{i \in [n]} \sum_{t_i > r} f(t_i)Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i +
      \alpha \sum_{i \in [n]} \Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i 
\end{align*}

We can think of $Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i$ as the expected revenue of the mechanisms that postes price $t_i$ on all items except the $i$-th item, but allows the buyer to get only one item.
Therefore $Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i\leq r$.
This implies:

\begin{align*}
      (\tail)
      \leq &
      \sum_{i \in [n]} \sum_{t_i > r} f(t_i)Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i +
      \alpha \sum_{i \in [n]} \Pr_{t \sim D}( t_{-i} \in \EE_{i,t_i})  \cdot t_i \\
    \leq &
    \sum_{i \in [n]} \sum_{t_i > r} f(t_i)r +
      n \alpha r \\
    \leq &
    \sum_{i \in [n]} \Pr_{t_i \sim D_i}[t_i > r] r +
      n \alpha r \\
    \leq & r (1 + n \alpha)
\end{align*}

\end{proof}

==> inaproximability_results.tex <==
%\section{Limitations of Approximation with Dobrushin Assumption}

\section{Missing Details from Section~\ref{sec:impossibility results}}\label{sec:appx_impossibility}
\argyrisnote{I moved the proof from this section to the main body}

\begin{prevproof}{Lemma}{lemma:mix_dobrushin}
Assume that $D=D_1\times D_2$, where $D_1$ and $D_2$ are the marginals of  $D'$. 
Let $T_i = \supp(D_i)$%=\supp(D_i')=\supp(D_i'')$
and $T= T_1 \times T_2$.
Let $A^{D'}=\{\alpha_{i,j}^{D'}\}_{i,j\in[2]}$ be the influence matrix of $D'$ and $A^{D''}=\{\alpha_{i,j}^{D''}\}_{i,j\in[2]}$ be the influence matrix of $D''$.
Note that the diagonal entries of $A^{D'}$ and of $A^{D''}$ are zero.
%We denote by $I_{j \rightarrow i}^D$  the influence from random variable $D_i$ to random variable $D_j$.
%Similarly we denote by $I_{j \rightarrow i}^{D''}$ the influence from random variable $D_i''$ to random variable $D_j''$.
We have that:
$$\alpha_{i,j}^{D''}
=  \max_{  \substack{ t_j,t'_j \in T_j } }  
	%
	d_{TV} \left( D''_{i \mid t_j},
	D''_{i \mid t_j'}\right) 
    = \alpha' \max_{ t_j,t'_j \in T_j  }  
	%
	d_{TV} \left( D'_{i \mid t_j},
	D'_{i \mid t_j'}\right) 
	= \alpha' \alpha_{i,j}^{D'}$$
\notshow{
\begin{align*}
\alpha_{i,j}^{D''}
= & \max_{  \substack{ t_j,t'_j \in T_j } }  
	%
	d_{TV} \left( D''_{i \mid t_j},
	D''_{i \mid t_j'}\right) \\
    = &\alpha' \max_{ t_j,t'_j \in T_j  }  
	%
	d_{TV} \left( D'_{i \mid t_j},
	D'_{i \mid t_j'}\right) \\
	=& \alpha' \alpha_{i,j}^{D'}
\end{align*}
}

In the statement of the lemma,
we assumed that $\alpha = ||A^{D'}||_\infty=\max(\alpha^{D'}_{1,2},\alpha^{D'}_{2,1})$.
We can easily infer the following: $||A^{D''}||_\infty = \max(\alpha_{1,2}^{D''},\alpha_{2,1}^{D''}) = \alpha' \max(\alpha_{1,2}^{D'},\alpha_{2,1}^{D'}) = \alpha' \cdot \alpha$. This concludes the fact that $D''$ has $\alpha(\vT) =\alpha' \cdot \alpha$.


Now we prove that $D''$ can be modeled as a MRF with finite inverse temperature.
We consider a MRF with potential functions $\psi_1(t_1) = 1,\forall t_1 \in T_1$, $\psi_2(t_2) = 1,\forall t_2 \in T_2$ and $\psi_{1,2}(\vT) = \ln\left( \Pr_{\vT' \sim D''}(\vT' =\vT)\right)$. Since Distribution $D''$ samples from the product distribution $D$ with probability $1-\alpha$,
we have that for each $\vT \in T$, {$\Pr_{\vT' \sim D''}(\vT' =\vT) \geq  (1-\alpha)p^2$. This is true because with probability $1-\alpha$ we sample from the product distribution $D$,
and with probability at least $p^2$ we sample the type $\vT$}, 
therefore the MRF we just described has finite inverse temperature {and $\Delta = \beta(\vT) = \max_{\vT \in \supp(D')} |\log\left(\Pr_{\vT' \sim D'}[\vT'=\vT] \right)|\leq |\log\left((1-\alpha)p^2 \right)|$}. In the case where the distribution is over two items, $\beta(\vT)= \max_{\vT \in T} |\psi_{1,2}(\vT)|$.
Moreover we can easily verify that the MRF we just described has the same joint distribution as $D''$.
Therefore $D''$ can be modeled as a MRF with finite inverse temperature.


We now prove that $\rev(D'') \geq \alpha' \rev(D')$.
This is true because we can simply use the optimal mechanism that induces $\rev(D')$ on $D''$.
Since $D''$ take a sample from $D'$ with probability $\alpha'$,
we are guaranteed that this mechanism has revenue at least $\alpha'\rev(D')$ on $D''$.

The fact that $D''$ has the same marginal distributions as $D'$ follows from the sampling procedure.
\end{prevproof}

\notshow{
In this section, we show that there exist MRFs that satisfy the Dobrushin uniqueness condition, while $\srev$ and $\brev$ cannot guarantee any multiplicative approximation of the optimal revenue.





First we present the main building block of our construction.


\begin{lemma}
\label{lemma:mix_dobrushin}
Let $D'$ be a correlated valuation distribution over $2$ items with $\alpha(\vT)=\alpha$.
Let $D$ be a product distribution that has the same marginal distributions as $D'$.
Then for any $0\leq \alpha' \leq 1$,
we consider the distribution $D''$ that takes a sample from $D'$ with probability $\alpha'$ and takes a sample from $D$ with probability $1-\alpha'$.
Distribution $D''$ can be modeled as a MRF with finite inverse temperature
{such that $\Delta = \beta(\vT) \leq |\log((1-\alpha) p^2)|$,
where $p = \inf_{\vT \in \supp(D')} \Pr_{\vT' \sim D'}[\vT'=\vT]$}%$(\beta(\vT) < +\infty)$
and $\alpha(\vT) = \alpha' \cdot \alpha$.
Furthermore, $D''$ has the same marginal distribution as $D$ and $\rev(D'') \geq \alpha'\rev(D')$.
\end{lemma}


\begin{proof}
Assume that $D=D_1\times D_2$, where $D_1$ and $D_2$ are the marginals of  $D'$.% = (D_1',D_2')$ and $D^{''}=(D_1^{''},D_2^{''})$.
Let $T_i = \supp(D_i)$%=\supp(D_i')=\supp(D_i'')$
and $T= T_1 \times T_2$.
Let $A^{D'}=\{\alpha_{i,j}^{D'}\}_{i,j\in[2]}$ be the $d$-Dobrushin interdependent matrix of $D'$ and $A^{D''}=\{\alpha_{i,j}^{D''}\}_{i,j\in[2]}$ be the $d$-Dobrushin interdependent matrix of $D''$,
under the trivial metric.
Note that the diagonal entries of $A^{D'}$ and of $A^{D''}$ are zero.
%We denote by $I_{j \rightarrow i}^D$  the influence from random variable $D_i$ to random variable $D_j$.
%Similarly we denote by $I_{j \rightarrow i}^{D''}$ the influence from random variable $D_i''$ to random variable $D_j''$.
We have that:

\begin{align*}
\alpha_{i,j}^{D''}
= & \max_{  \substack{ t_j,t'_j \in T_j } }  
	%
	d_{TV} \left( D''_{i \mid t_j},
	D''_{i \mid t_j'}\right) \\
    = &\alpha' \max_{ t_j,t'_j \in T_j  }  
	%
	d_{TV} \left( D'_{i \mid t_j},
	D'_{i \mid t_j'}\right) \\
	=& \alpha' \alpha_{i,j}^{D'}
\end{align*}

In the statement of the lemma,
we assumed that $\alpha = ||A^{D'}||_\infty=\max(\alpha^{D'}_{1,2},\alpha^{D'}_{2,1})$.
We can easily infer the following.

\begin{align*}
    ||A^{D''}||_\infty = \max(\alpha_{1,2}^{D''},\alpha_{2,1}^{D''}) = \alpha' \max(\alpha_{1,2}^{D'},\alpha_{2,1}^{D'}) = \alpha' \cdot \alpha
\end{align*}

This concludes the fact that $D''$ has $\alpha(\vT) =\alpha' \cdot \alpha$.


Now we prove that $D''$ can be modeled as a MRF with finite inverse temperature.
We consider an MRF with potential functions $\psi_1(t_1) = 1,\forall t_1 \in T_1$, $\psi_2(t_2) = 1,\forall t_2 \in T_2$ and $\psi_{1,2}(\vT) = \ln\left( \Pr_{\vT' \sim D''}(\vT' =\vT)\right)$. Since Distribution $D''$ samples from the product distribution $D$ with probability $1-\alpha$,
we have that for each $\vT \in T$, {$\Pr_{\vT' \sim D''}(\vT' =\vT) \geq  (1-\alpha)p^2$. This is true because with probability $1-\alpha$ we sample from the product distribution $D''$,
and with probability at least $p^2$ we sample the type $\vT$.},
therefore the MRF we just described has finite inverse temperature {and $\Delta = \beta(\vT) = \max_{\vT \in \supp(D')} |\log\left(\Pr_{\vT' \sim D'}[\vT'=\vT] \right)|\leq |\log\left((1-\alpha)p^2 \right)|$}. In the case where the distribution is over two items, $\beta(\vT)= \max_{\vT \in T} |\psi_{1,2}(\vT)|$.
Moreover we can easily verify that the MRF we just described has the same joint distribution as $D''$.
Therefore $D''$ can be modeled as an MRF with finite inverse temperature.


We now prove that $\rev(D'') \geq \alpha' \rev(D')$.
This is true because we can simply use the optimal mechanism that induces $\rev(D')$ on $D''$.
Since $D''$ take a sample from $D'$ with probability $\alpha'$,
we are guaranteed that this mechanism has revenue at least $\alpha'\rev(D')$ on $D''$.

The fact that $D''$ has the same marginal distributions as $D'$ follows from the sampling procedure.
\end{proof}


Now we present an important result from \cite{HARTN_2019}.

\begin{lemma}[Theorem~A from \cite{HARTN_2019}]
\label{lemma:bad_distribution}
For any positive real number $N$, there exists a two item correlated distribution $D$,
such that for an additive buyer whose type is sampled from $D$, $\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}>N$.
%$\brev(D)=O(1)$ and $\srev(D) = O(1)$, while $\rev(D)>N$.
\end{lemma}

Now we are ready to present the  inapproximability result.




\begin{prevproof}{Theorem}{lem:inaprx_dob}
Let $D'$ be the distribution over two items that is guaranteed to exist by Lemma~\ref{lemma:bad_distribution}. Since $D'$ is a two dimensional distribution, its Dobrushin coefficient is at most $1$.


Apply Lemma~\ref{lemma:mix_dobrushin} to $D'$ with parameter $\alpha'=\alpha$ to create another distribution $D$ which has the same marginals as $D'$ but with a Dobrushin coefficient at most $\alpha$. Moreover, $D$ can be expressed as an MRF with finite inverse temperature. Clearly, $\rev(D)\geq \alpha\cdot \rev(D')$, as one can simply achieve the LFS using the optimal mechanism designed for $D'$. Also, $\srev(D')=\srev(D)$ as the two distributions have the same marginals. Finally, $\brev(D')\leq 2\srev(D')$. Suppose $b$ is the optimal price for the bundle, then we can set the two items separately each at price $b/2$. Clearly, whenever the bundle is sold, at least one item is sold. To conclude, $$\frac{\rev(D)}{\max\{\brev(D),\srev(D)\}}\geq \frac{\rev(D)}{2\srev(D)}\geq \frac{\alpha\cdot\rev(D')}{2\srev(D')}>\frac{\alpha}{2}\cdot N.$$
%we can generate a type distribution generated by a MRF $D'$ such that $\alpha(\vT) \leq \alpha$, has finite inverse temperature and has the same marginal distributions as $D$. Since the $\rev(D)$ can be arbitrary high, for a fixed value of $\alpha$ we can also make sure that $\rev(D') \geq \alpha\rev(D)$ is also arbitrary high.


%Since we assume that the agent has additive valuation, $\bm{SRev}(D')$ only depends on the marginal distribution of $D'$. Therefore since $D$ and $D'$ have the same marginal distributions,
%$\bm{SRev}(D')=\bm{SRev}(D)=O(1)$. We now prove that $\bm{BRev}(D') \leq 2\bm{SRev}(D)= O(1)$. Suppose $B$ is the posted price on the grand bundle. If we sell each item separately at price $B/2$, then we have revenue at least $\bm{BRev}/2$,so $\bm{SRev} \geq \bm{BRev}/2$. Therefore $\bm{SRev}=\bm{BRev}=O(1)$. This concludes our proof.
\end{prevproof}
}


%Lemma~\ref{lem:inaprx_dob} implies that even if we consider buyers type valuation that are generated by a MRF that satisfy the Dobrushin Uniqueness Condition, the revenue of simple mechanisms cannot be bounded by a multiplicative or additive term that depends on the value of $\alpha(\vT)$. A valid multiplicative or approximation bound should also include other parameters of the problem (like the inverse temperature).


























%
%
%
%
%
%
%
%
%
%
%


==> spectra_metric_fast_mixing.tex <==
\section{Bounded Spectral Radius of d-Dorbushin Interdependent Matrix implies Fast Mixing}

First we provide a necessary definition.

\begin{definition}[Definition~2,3 \cite{Hayes06}]
Consider a distribution $D$ over $n$ items.
The Glauber Dynamics of $D$ is a Markov Chain whose set of states is $T=\supp(D)$.
Now we define how the transition between states happen.
Suppose we are at state $\vT \in T$ at time $t$,
first we sample an item $i^*$ uniformly at random among the $n$ items,
then we take a sample $t_s$ from $D_{i^* \mid \vT_{-i^*}}$ and transit to $\vT'$:

\begin{align*}
    \vT'_i =
    \begin{cases}
    t_s \quad &\text{if $i=i^*$} \\
    t_i & \text{o.w.}
    \end{cases}
\end{align*}
\end{definition}

Consider a distribution $D$ over $n$ items.
Hayes showed that if the spectral radius of the Dobrushin Interdependent Matrix (which is the $d$-Dobrushin interdependent matrix, where $d(x,y)=\mathds{1}[x \neq y]$) of $D$ is less than $1$,
then we are guaranteed fast mixing time \cite{Hayes06}.
We are going to extend his results and prove that if there exists a metric $d(\cdot,\cdot):E \times E \rightarrow \mathbb{R}$,
such that the spectral radius of $d$-Dobrushin interdependent matrix of $D$ is less than $1$,
then we are guaranteed fast mixing time.
We make this statement formal in the following lemma.
Our proof is based on proof of Theorem~6 in \cite{Hayes06}.

\begin{lemma}\label{lemma:rapid mixing}
Let $D$ be a distribution over $n$ items (not necessarily a MRF) and $T=\supp(D)$.
Let $(E,d)$ be a metric space, where $E= \cup_{i\in[n]}T_i$.
Let $\rho$ be the spectral radius of the $d$-Dobrushin interdependent matrix of $D$.
If $\rho < 1$,
then the mixing time of Glauber Dynamics of $D$ is $O\left(\frac{n}{1-\rho}\log \left(n\frac{\sup_{\vT,\vT' \in E}d(\vT,\vT')}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} \right) \right)$.
\end{lemma}




\begin{proof}
Let $A$ be the $d$-Dobrushin Interdependent matrix of $D$.
Let \argyrisnote{$(X^0=(X^0_1,\ldots,X^0_n),Y^0=(Y^0_1,\ldots,Y^0_n)) \in T\times T$} and $(X^t,Y^t)_{t\geq 0}$ be the evolution of Glauber Dynamics when the chains start at $(X^0,Y^0)$,
where \argyrisnote{$X^t=(X_1^t,\ldots,x_n^t),Y^t=(Y^t_1,\ldots,Y^t_n)$} have the following coupling.

Suppose we are at time step $t$ and our Glauber Dynamics are at states $(X^t,Y^t)$.
For the next step, we first sample an item $i^*$ uniformly at random among the $n$ items and
then we use a coupling that minimizes the value of $\E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid \text{item $i^*$ was chosen  to be updated}\right]$.


We are going to prove the following inequality using the Path Coupling technique.
\argyrisnote{
\begin{align*}
    \E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid X^t,Y^t, \text{item $i^*$ was chosen to be updated} \right] \leq \sum_{j \in [n]} \alpha_{i^*,j} d\left(X^t_j,Y^t_j\right)
\end{align*}
}

We consider the following auxiliary random variables \argyrisnote{$\left(Z^i=(Z^i_1,\ldots,Z^i_n)\right)_{0 \leq i \leq n}$} in the Glauber Dynamics setting.
Let $Z^0=X^t$ and for $i\geq 1$:
\begin{align*}
Z^i_j =
\begin{cases}
Y^{t}_j \quad &\text{ if $j = i$ } \\
Z^{i-1}_j \quad &\text{ o.w. }
\end{cases}
\end{align*}

Note that $Z^i$ and $Z^{i+1}$ may differ only in the type of the $i+1$ item and that $Z^n = Y^t$.
\argyrisnote{Let $W^i=(W^i_1,\ldots,W^i_n)$ be the position of Glauber Dynamics starting at state $Z^i$ after one step according to the coupling we are going to describe now.}
%
\argyrisnote{We first sample an item $i^*$ uniformly at random among the $n$ items and
for all $i\in[n]$, in $W^i$ we choose to update the type for item $i^*$.}
%
Since $d$ is a metric, we have the following:
%
\begin{align*}
\E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid X^t,Y^t, \text{item $i^*$ was chosen} \right] \leq   \E\left[ \sum_{j \in \left[n\right]} d\left(W^{j-1}_{i^*},W^{j}_{i^*}\right) \mid \land_{0\leq i\leq n} Z^i, \text{item $i^*$ was chosen}\right]
\end{align*}


Now we describe how we couple the value of $W_{i^*}^j$ by induction.
First we randomly sample the value of $W_{i^*}^0$ from $D_{i^* \mid X^t_{-i^*}}$.
\argyrisnote{Now suppose we have sampled the value of $W_{i^*}^{j-1}$,
we take a sample of $W_{i^*}^i$ with a coupling such that $E\left[ d\left(W^{j-1}_{i^*},W^{j}_{i^*}\right) \mid Z^{j-1},Z^j, \text{item $i^*$ was chosen}\right] \leq \alpha_{i^*,j} d\left(Z^{j-1}_j,Z^{j}_j\right)=\alpha_{i^*,j} d\left(X^t_{j},Y^{t}_{j}\right)$.}
Such a coupling is guaranteed to exist by definition of the $d$-Dobrushin interdependent matrix.


Since we assumed that the coupling between $X^{t+1}_{i^*}$ and $Y^{t+1}_{i^*}$ minimizes the expected value of $\E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \right]$, conditioned on the fact that the type of item $i^*$ was chosen to be updated,
we can infer that:

\begin{align*}
    \E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid X^t,Y^t\right] \leq &   \E\left[ \sum_{j \in \left[n\right]} d\left(W^{j-1}_{i^*},W^{j}_{i^*}\right) \mid \land_{0\leq i\leq n} Z^i, \text{item $i^*$ was chosen}\right] \\
    \leq & \sum_{j \in \left[n\right]} \alpha_{i^*,j} d\left(X^t_{j},Y^{t}_{j}\right)
\end{align*}

We also note the following:

\begin{align*}
    \E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid X^t,Y^t, \text{item $i^*$ was not chosen} \right] = d\left(X^t_{i^*},Y^t_{i^*}\right) 
\end{align*}

By combining the previous two inequalities,
we can conclude that:

\begin{align*}
    \E\left[ d\left(X^{t+1}_{i^*},Y^{t+1}_{i^*}\right) \mid X^t,Y^t \right] =\frac{n-1}{n} d\left(X^t_{i^*},Y^t_{i^*}\right)  + \frac{1}{n}\sum_{j \in [n]} \alpha_{i,j} d\left(X^t_j,Y^t_j\right)
\end{align*}

Let $d^t=\left(d(X^t_1,Y^t_1),\ldots, d(X^t_n,Y^t_n)  \right)$.
Let $I$ be the $n\times n$ identity matrix.
We can infer that:


\begin{align*}
    \E\left[d^{t+1} \mid X^t,Y^t\right] \leq \left( \frac{n-1}{n}I + \frac{1}{n}A \right)d^t
\end{align*}


By Law of Total Expectation we have that:

\begin{align*}
    \E\left[d^{t+1} \right] \leq \left( \frac{n-1}{n}I + \frac{1}{n}A \right)\E[d^t]
\end{align*}

Thus:

\begin{align*}
    \E\left[d^{t+1} \right] \leq \left( \frac{n-1}{n}I + \frac{1}{n}A \right)^{t+1}\E[d^0]
\end{align*}


Let $B=\frac{n-1}{n}I + \frac{1}{n}A$,
then $||B||_2 = 1 - \frac{1-\rho}{n}$.
Note that $\Pr\left[X^t_i \neq Y^t_i \right]=\Pr\left[d\left(X^t_i , Y^t_i\right) \geq \inf_{\vT \neq \vT' \in E}d(\vT,\vT') \right] \leq \frac{\E\left[ d\left(X^t_i \neq Y^t_i\right) \right]}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')}$,
where in the last step we used Markov Inequality.
We have that:

\begin{align*}
    d_{TV}\left(X^t , Y^t \right) \leq \Pr\left[ X^t \neq Y^t \right] \leq & \frac{||d^t||_1}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} \\
    \leq & \frac{\sqrt{n}}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} ||d^t||_2 \\
    \leq & \frac{\sqrt{n}}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} ||B^t d^0||_2 \\
    \leq & \frac{\sqrt{n}}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} ||B||_2^t ||d^0||_2 \\
    \leq & \frac{\sqrt{n}}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} ||B||_2^t \sqrt{n}\sup_{\vT,\vT' \in E}d(\vT,\vT') \\
    = & \frac{\sup_{\vT,\vT' \in E}d(\vT,\vT')}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} n\left( 1 - \frac{1-\rho}{n} \right)^t 
\end{align*}

Therefore if we set $T(\delta)= \frac{n}{1-\rho}\log \left(\frac{\sup_{\vT,\vT' \in E}d(\vT,\vT')}{\inf_{\vT \neq \vT' \in E}d(\vT,\vT')} \frac{n }{\delta} \right)$,
we have that $d_{TV}\left(X^{T(\delta)} , Y^{T(\delta)} \right) \leq \delta$ which concludes the proof.
\end{proof}






==> usefuless_dobrushin.tex <==

{\color{red}
------This section states that if we do not make any assumption about the Dobrushin Condition of a distribution,
then Brev could be the same as Srev.


If we make an assumption about the Dobrushin condition of the distribution,
then Brev concentrates better
--------

\subsubsection{Usefulness of Dobrushin Coefficient}

Inspired by \cite{BabaioffILW14}.


Let $D$ be an an arbitrary distribution over $n$ items,
such that the marginal distribution of each item $i$, is the Equal Revenue Distributions.
First, we note that $\srev=n$.
Now we are going to show that if we don't make any assumption about the Dobrushin coefficient of $D$,
then $\brev$ could almost equal to the welfare.



\begin{lemma}[Inspired by \cite{BabaioffILW14}.]
Let $D$ be an additive type distribution over $n$ items,
such that the marginal distribution of the value of each item $i$, is the Equal Revenue Distributions.
There is a valid instance of distribution $D$ such that $\brev=n$.
\end{lemma}

\begin{proof}
We denote by $ER$ the Equal revenue distribution.
We consider the following distribution $D$.
First we sample $t$ from $ER$ and we output $(t,t,\ldots,t)$.
We note that the marginal distribution for each item $i$ is the Equal Revenue Distribution.
Now that we have defined the distribution $D$,
we are going to calculate the $\brev$ induced by this distribution.
We are going to calculate the revenue of the grand bundle at price $p$.

\begin{align*}
     p \Pr_{\vT \sim D}\left[ \sum_i t_i \geq p \right] =& \Pr_{t \sim ER}\left[ n \cdot t \geq p \right] \\
    =& p\Pr_{t \sim ER}\left[  t \geq \frac{p}{n} \right] \\
    =& \frac{p\cdot n}{p} \\ =& n
\end{align*}

Which implies that $\brev$ is also equal to $n$.

\end{proof}





The following Lemma provides us with a concentration inequality that we need.


\begin{lemma}[Theorem~4.3 in\cite{chatterjee2005concentration}\cite{C2005,D19,K2003}]
\label{lemma:dobrushin_concentration}
For any distribution $D$ over $n$ random variables that has Dobrushin coefficient $\alpha$ and function $f$ with the bounded differences property with parameters $c_1,c_2,\ldots,c_d$,
then we have that:

\begin{align*}
    \Pr_{t\sim D}\left[\left|f(t) - \E_{t \sim D}[f(t)]\right|\geq p\right] \leq 2e^{-\frac{(1-\alpha)p^2}{2\sum_{i=1}^d c_i^2}}
\end{align*}


\end{lemma}



\begin{lemma}
Let $D$ be an additive type distribution over $n$ items that has Dobrushin Coefficient $\alpha<1$.
If the marginal distribution of the value of each item $i$ is the Equal Revenue Distribution supported on  $[1,\sqrt{n(1-\alpha)}]$ and $n= \Omega \left(\frac{1}{1-\alpha}\right) $
then $\brev= O\left( n\log(n(1-\alpha) ) \right)$ and welfare $O\left( n\log(n(1-\alpha) ) \right)$
\end{lemma}

\begin{proof}
We denote by $ER$ the equal revenue distribution.
We consider the additive valuation function $f(\vT):\left[0,\sqrt{n(1-\alpha)}\right]^n \rightarrow \mathbb{R}$ such that $f(\vT) = \sum_i t_i$.
This implies that $f(\vT)$ has the bounded difference property with parameters $c_i = \sqrt{n(1-\alpha)}$.
By Linearity of expectation,
we have that the welfare of $D$ is equal to $\E_{t\sim D}[f(\vT)] = n E_{t\sim ER}[t]=n \left( \frac{\ln(n(1-\alpha))}{2} + 1 \right)$.
Using Lemma~\ref{lemma:dobrushin_concentration} with $p=n\sqrt{2 \ln(4)}$,
we have from  that:

\begin{align*}
        & \Pr_{\vT \in D}\left[f(\vT) \leq \E_{\vT \sim D}[f(\vT)]| -  p\right] \leq 2e^{-\frac{(1-\alpha)p^2}{2\sum_{i=1}^d c_i^2}} \\
        \Leftrightarrow &
        \Pr_{\vT \sim D}\left[f(\vT) \leq \frac{n\ln(n(1-\alpha))}{2} + n  -  n\sqrt{2 \ln(4)}\right] \leq \frac{1}{2}
\end{align*}

This statement implies that with probability at least $\frac{1}{2}$,
we sell the grand bundle at price $\frac{n\ln(n(1-\alpha))}{2} - n \left( \sqrt{2 \ln(4)} - 1 \right)$.
Therefore:

\begin{align*}
    \brev \geq \left( \frac{n\ln(n(1-\alpha))}{2} - n \left( \sqrt{2 \ln(4)} - 1 \right) \right)
    \cdot \frac{1}{2} = O \left( n \ln(n(1-\alpha)) \right)
\end{align*}

Which concludes the proof.
\end{proof}



}


\begin{comment}

\begin{proof}
First we are going to bound the covariance between random variable $t_i$ and $t_j$ where $i\neq j$.



First, we note that term (CORE) is the expected value for the grand bundle that a buyer has when each of her coordinates is less or equal than $S_{rev}$.


By Lemma~\ref{lemma:dobrushin_concentration} we have that with probability at least $1-2e^{-(1-\alpha)\beta^2}$,
the value for the grand bundle of a buyer is between $E[f(z)] - \sqrt{2}\beta S_{Rev}$ and $E[f(z)] + \sqrt{2}\beta S_{Rev}$.
Therefore if wet a a price for the grand bundle of value $E[f(z)] - \sqrt{2}\beta S_{Rev}$,
then the buyer get the bundle with probability at least $1-2e^{-(1-\alpha)\beta^2}$ and the difference between the value of the grand bundle from the buyer and the revenue is at most:
\begin{align*}
   2\sqrt{2}\beta S_{Rev}
\end{align*}

We can assume that with probability at most $2e^{-(1-\alpha)\beta^2}$,
our Grand Bundle price, lose $S_{Rev}$ from the expected welfare.
Therefore we have that:

\begin{align*}
CORE \leq & B_{Rev}+ 2\sqrt{2}\beta S_{Rev}\left(1- 2e^{-(1-\alpha)\beta^2} \right)  + S_{Rev}\cdot 2e^{-(1-\alpha)\beta^2} \\
= & B_{Rev} + 2S_{Rev}\left( \sqrt{2}\beta - (2\sqrt{2}\beta - 1)e^{-(1-\alpha)\beta^2} \right)
\overset{\left( \beta = \frac{1}{2\sqrt{2}} \right)}{=} B_{Rev}+S_{Rev}
\end{align*}


\end{proof}

\end{comment}
